Deception by Omission: Using Adversarial Missingness to Poison Causal Structure Learning

Inference of causal structures from observational data is a key component of causal machine learning; in practice, this data may be incompletely observed. Prior work has demonstrated that adversarial perturbations of completely observed training data may be used to force the learning of inaccurate causal structural models (SCMs). However, when the data can be audited for correctness (e.g., it is crytographically signed by its source), this adversarial mechanism is invalidated. This work introduces a novel attack methodology wherein the adversary deceptively omits a portion of the true training data to bias the learned causal structures in a desired manner. Theoretically sound attack mechanisms are derived for the case of arbitrary SCMs, and a sample-efficient learning-based heuristic is given for Gaussian SCMs. Experimental validation of these approaches on real and synthetic data sets demonstrates the effectiveness of adversarial missingness attacks at deceiving popular causal structure learning algorithms.

==> experiments/table_sachs_sim.tex <==
% Table generated by Excel2LaTeX from sheet 'edit'
\begin{table}[htbp]
	\centering
	\caption{Results for the ``Sachs Simulation'' experiment. Average results of 20 random mask samples.}
	\resizebox{1\columnwidth}{!}{%
		% Table generated by Excel2LaTeX from sheet 'sachs sim'
\begin{tabular}{|l|c|r|r|r|r|}
\toprule
\multicolumn{1}{|c|}{\multirow{2}[4]{*}{Modeler}} & \multirow{2}[4]{*}{Initial.} & \multicolumn{2}{c|}{MNAR (NN)} & \multicolumn{2}{c|}{MCAR} \\
\cmidrule{3-6}      &       & \multicolumn{1}{l|}{HD($\hat{\mathcal{G}},\mathcal{G}_{p}$)} & \multicolumn{1}{p{5em}|}{ Success} & \multicolumn{1}{l|}{HD($\hat{\mathcal{G}},\mathcal{G}_{p}$)} & \multicolumn{1}{p{5em}|}{ Success} \\
\midrule
\multicolumn{1}{|c|}{\multirow{5}[10]{*}{MissDAG}} & \multicolumn{1}{l|}{Emp. Diag.} & 15.25 & 0.85  & 13.95 & 0.25 \\
\cmidrule{2-6}      & \multicolumn{1}{l|}{IW(*)} & 15.2  & 0.8   & 14.15 & 0.4 \\
\cmidrule{2-6}      & \multicolumn{1}{l|}{Ident.} & 15.2  & 0.8   & 13.9  & 0.25 \\
\cmidrule{2-6}      & \multicolumn{1}{l|}{Random(*)} & 15.2  & 0.8   & 13.8  & 0.25 \\
\cmidrule{2-6}      & \multicolumn{1}{l|}{True} & 15.3  & 0.9   & 14    & 0.2 \\
\midrule
MissPC & -     & 12.1  & 1     & 10.05 & 0.05 \\
\midrule
Mean + NT & -     & 15.35 & 1     & 14.95 & 0.55 \\
\midrule
Mean + PC & -     & 12.05 & 0.95  & 10.15 & 0 \\
\bottomrule
\end{tabular}%

	}
	\label{tab:addlabel}%
\end{table}%


==> source.tex <==
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{bm}
\usepackage{caption}
\usepackage{verbatim}
\usepackage{enumitem}

% hyperref makes hyperlinks in the resulting PDF.
\usepackage{hyperref}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% For theorems and such
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{amsthm}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}

\usepackage{algorithm}
\usepackage{algorithmic}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
\usepackage[disable,textsize=tiny]{todonotes}
%\usepackage[textsize=tiny]{todonotes}

\input{math_commands}
\input{denizMath}
\def\independent{\perp \!\!\! \perp}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\p}{\mathrm{p}}
\renewcommand{\E}{\mathbb{E}}
\renewcommand{\vx}{\mathbf{x}}
\renewcommand{\rvx}{\mathbf{X}}
\renewcommand{\that}{\hat{\bm{\theta}}}
\renewcommand{\vtheta}{\bm{\theta}}
\renewcommand{\rvr}{\mathbf{R}}
\renewcommand{\rv}{\mathbf{r}}
\renewcommand{\pa}{\mathrm{pa}}
\newcommand{\anc}{\mathrm{anc}}

\usepackage{multirow}
\usepackage{booktabs}
\usepackage{colortbl}

\begin{document}
%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.
\title{Deception by Omission:\\ Using Adversarial Missingness to Poison Causal Structure Learning}

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.


%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.

%\renewcommand{\shortauthors}{Koyuncu, Gittens, Yener, and Yung}

%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}
  Causality-informed machine learning has been proposed as an avenue for achieving many of the goals of modern machine learning, from ensuring generalization under domain shifts to attaining fairness, robustness, and interpretability. A key component of causal machine learning is the inference of causal structures from observational data; in practice, this data may be incompletely observed. Prior work has demonstrated that adversarial perturbations of completely observed training data may be used to force the learning of inaccurate causal structural models (SCMs). However, when the data can be audited for correctness (e.g., it is crytographically signed by its source), this adversarial mechanism is invalidated. This work introduces a novel attack methodology wherein the adversary deceptively omits a portion of the true training data to bias the learned causal structures in a desired manner (under strong signed sample input validation, this behavior seems to be the only strategy available to the adversary). Under this model, theoretically sound  attack mechanisms are derived for the case of arbitrary SCMs, and a sample-efficient learning-based heuristic is given. Experimental validation of these approaches on real and synthetic data sets demonstrates the effectiveness 
of adversarial missingness attacks at deceiving popular causal structure learning algorithms.
\end{abstract}

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%

\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147</concept_id>
<concept_desc>Computing methodologies</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010178</concept_id>
<concept_desc>Computing methodologies~Artificial intelligence</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010257.10010293</concept_id>
<concept_desc>Computing methodologies~Machine learning approaches</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10002978</concept_id>
<concept_desc>Security and privacy</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies}
\ccsdesc[500]{Computing methodologies~Artificial intelligence}
\ccsdesc[500]{Computing methodologies~Machine learning approaches}
%\ccsdesc[500]{Security and privacy}



%%%




%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{Causal ML, Causal Structure Learning, Missing Data, Adversarial ML}


\received{20 February 2007}
\received[revised]{12 March 2009}
\received[accepted]{5 June 2009}

%%
%% This command processes the author and affiliation and title
%% information and builds the first part of the formatted document.
\maketitle



\section{Background} 

 A \emph{causal factorization} of the distribution $\P$ of a random $d$-dimensional vector $\rvx$ explicitly identifies the causes of each variable $\rvx_i$, in the form
 \[
 \P_\rvx = \prod_{i=1}^d \P_{\rvx_i \mid \rvx_{\pa_i} },
 \]
 where $\pa_i$ denotes the indices of the parents of variable $\rvx_i$ in an associated directed acyclic graph (DAG) $\mathcal{G}$.  When $\P$ has a causal factorization corresponding to $\mathcal{G}$, it is \emph{Markovian} with respect to $\mathcal{G}$:  conditioned on its parents, each $\rvx_i$ is independent of its non-descendants. Conversely, $\P$ is said to be \emph{faithful} with respect to $\mathcal{G}$ if every conditional independence in $\P$ is encoded in $\mathcal{G}$.
 
 A structural causal model (SCM) associated with $\mathcal{G}$ expresses the cause-effect relationships using functional relations of the form
 \[
\rvx_i := f_i(\rvx_{\pa_i}, \rvn_i),
 \] 
 indicating that each variable is determined by the values of its parent variables, and a noise variable $\rvn_i$.
 Here, the exogenous noise variables $\rvn_1, \ldots, \rvn_d$ are assumed to be jointly independent of each other and the endogenous variables $\rvx$. 

%\subsection{Causal Learning}
 %Causal reasoning uses the causal factorization of $\P$ and involves the three levels of causal reasoning: (i) \emph{observational reasoning}, corresponding to simple statements about $\P$ such as $\P[\vy=y\,|\,\vx_6=x]$ (i.e., probability of a particular loan default conditional on a specified amount of debt), (ii) \emph{interventional reasoning} such as $\P[\vy=y\,|\,\text{do}(\vx_6=x)]$, corresponding to statements about the joint distribution that results from forcibly modifying one of random variables $\vx_i$ and allowing its changes to propagate through to alter the distribution of the other variables according to the causal factorization, i.e. $\P[\vx=(x_1, \ldots,x_p) \,|\, \text{do}(\vx_i = x)] = \prod_{j=1, j \neq i}^p \P[\vx_j = x_j \,|\, \text{PA}_j] \delta_{\vx_i = x}$, and (iii) \emph{counterfactual reasoning}, which in essence allows you to specify a ``universe" in which observations $\vx_i$ were made, by constraining the values of the $\vn_i$ to be consistent with those observations, then to answer interventional questions in this universe, for example $\P[\vy=y\,|\,\vx_2=z, \text{do}(\vx_6=x)]$.%\footnote{The simplified notation employed here is ambiguous in that it does not distinguish between counterfactual distributions and conditioned counterfactual distributions, e.g. one in which the counterfactual universe $\vx_2 = z, \text{do}(\vx_6 = x)$ is then conditioned on the observation $\vx_6 = x$. Conditioned counterfactual distributions do not appear in this paper.}. 
  
% Observational, interventional, and counterfactual distributions are generically not equivalent. For example, observing $\vx_6$ constrains the likely values of $\vx_5$ because $\vx_6$ is an effect of $\vx_5$, which in turn affects the probability that $\vy=y$ because it is a child of both $\vx_5$ and $\vx_6$; by contrast, intervening to set $\vx_6 = x$, does not affect the value of $\vx_5$, so the intervention and observations lead to different probabilities i.e. $\P[\vy=y\,|\,\vx_6=x] \neq \P[\vy=y\,|\,\text{do}(\vx_6=x)].$ Similarly, if we are in a universe where $\vx_2 = 2$, then the value of $\vx_5$ is constrained as a child of $\vx_2$, so observing that $\vx_2 = 2$ and then intervening on $\vx_6$ affects the probability that $\vy=y$ in a different manner than simply intervening on $\vx_6$, i.e. $\P[\vy=y\,|\,\text{do}(\vx_6=x)] \neq \P[\vy=y\,|\,\vx_2=z, \text{do}(\vx_6=x)]. $ 

 % Observational reasoning requires only knowledge of $\P$. Interventional reasoning requires at least a causal factorization of $\P$. Counterfactual reasoning requires an SCM, to enable the following steps~\cite{pearl2009causality}: \emph{abduction}, in which a posterior distribution on $\vn$ is computed given the evidence, \emph{action}, in which the structural equations are modified according to the given intervention, then \emph{prediction} in which the distribution of the non-intervened variables are computed using the posterior on $\vn$ and the modified structural equations.


 % \subsection{Causal Structure Learning}
 % \todo{Write section: emphasize in principle need observational and interventional data. Classic approachs (PC alg, and I think the score matching for Gaussian SCMs) learn partially directed graphs and direct ambiguous edges using interventional experiments. Practically speaking can be too expensive to get interventional data or more observational data, so recent emphasis in literature is on algorithms that work with observational data only to learn DAGs. Give refs to classic and modern algorithms to confirm these claims. Mention here the SHD as common metric used to measure recovery.}
  

  \subsection{Causal Structure Learning}
%  \todo{fill in this section}
%  \todo{BY: Alex did you delete some text I used to fill this section?}
%  \todo{dk:at least PC algorithm should be added}
  Causal networks arise naturally in a wide variety of application domains, including genetics,
epidemiology, and time series analysis. Learning causal structures from data is useful in these domains and others to facilitate principled interventional and counterfactual reasoning. Further, causal structures have become popular in machine learning, where they have been used successfully to tackle many of the difficult challenges that plague purely statistical machine learning, such as generalization under distribution shifts, adversarial robustness, and interpretability.
  
  A recent approach to causal discovery uses differentiable formulations of the DAG constraint. The original such algorithm, called NOTEARS~\cite{notears}, minimizes the residuals resulting from the linear SCM with a differentiable constraint encouraging the fitted model to be Markov relative to a DAG. This formulation is equivalent to maximizing the log-likelihood of an equal variance linear Gaussian model with a DAG constraint~\cite{golem}.


 \subsection{Missing Data}

In practical problems, including in causal discovery problems, missing data is a common issue. When missing data is present, standard causal structure learning algorithms cannot be used: direct application of structure learning algorithms using samples containing structured missingness may result in the learning of incorrect structures, e.g. due to selection bias. Instead, algorithms that learn structure from missing data must estimate the full data distribution from the incompletely observed data. 

Missing data problems are studied under three basic models: (i) Missing Completely at Random (MCAR), (ii) Missing at Random (MAR), and (iii) Missing Not At Random (MNAR). In the MCAR model, the distribution of the missingness is independent of that of the features, while in the MAR model, the missingness depends at most on the observed features. In the most general model, MNAR, the missingness may depend on both the observed and unobserved features. Most algorithms with provable properties for dealing with missing data require the MCAR or MAR assumptions.

There are recent results on causal discovery in the presence of non-adversarial missing data.
\cite{tu2019causal,thoemmes2015graphical,bhattacharya2020identification,10.5555/3020847.3020930,mohan2014graphical}.
%\todo{give more details on these references and their approaches, say how modern approaches allow DAGs from missing data, while others (e.g. Missing value PC) give CPDAGs. Mention approaches relevant to linear Gaussian SCMs with missing data. Emphasize these approaches seem to apply in MAR, and it is recommended when don't have a model of missingness that MAR should be used.}
%\todo{dk: 1. missPC should be explained, 2. MAR assumption should be supported}
MissDAG \cite{missdag} and MissGLasso \cite{MissGLasso2010} follow the same recipe for extending existing structure learning algorithms into the missing data setting. Both propose to maximize the log-likelihood of the observed data assuming the missigness mechanism is ignorable. Next, both use the EM algorithm to maximize a lower bound iteratevely. In MissGLasso, the maximization step contains the graphlasso \cite{graphlasso} penalty on the precision matrix and can be solved exactly. While in MissDAG, the maximization step contains a DAG constraint (plus a sparsity penalty) and can only be solved approximately with for example the NOTEARS algorithm.

\subsection{Adversarial Attacks on Causal Discovery}
 A large body of work has arisen around data poisoning, presenting new attacks and defenses~\cite{dai2019backdoor,liu2018fine,fang2020influence} in applications ranging from text classification to image recognition models to recommendation systems. Attacks on causal discovery have only recently been investigated as an instance of data poisoning via insertion of adversarial samples~\cite{alsuwat2018cyber,alsuwat2020adversarial}. Both of these works consider the problem of adding data to the training set in order to influence the causal structures learned by the classical PC algorithm~\cite{spirtes2000causation}, and demonstrate the feasibility of both targeted and untargeted attacks.
To our knowledge, no prior work has considered the use of missingness, rather than the insertion of false data, to manipulate the causal discovery process.

%\todo{where do we put the modeler's objective}

\section{Formulation of Adversarial Missingness}
\label{sxn:formulation}
To design adversarial attacks on the modeler that are effective, we assume that the objective which the modeler uses to find the causal structure from missing data is known. We make two assumptions: (i) the modeler assumes that the missingness mechanism is MAR, and (ii) the modeler finds the causal structure that maximizes the probability of the partially observed data. The first assumption is justified by the use of the MAR assumption in several approaches to learning causal structure from incompletely observed data. 

The second is assumption is justified by noting that in the case where the training data is completely observed, a common approach for the modeler is to learn a causal structure that maximizes the probability of the fully observed data subject to the distribution factorizing according to a DAG:
\begin{equation*}\label{eq:full}
	\that = \argmax_{\vtheta \in \mathcal{D} } \E_{\rvx; \vtheta_p}[ \log \P_{\rvx}(\vx;\vtheta) ].
\end{equation*}
Here, the distribution $\P_\mathbf{X}(\cdot; \vtheta)$ is from a parameterized family, and $\mathcal{D}$ is the set of parameters which satisfy the property that the corresponding distribution factorizes according to a DAG. 

%\todo{give references for this approach, or justify it.}
%\todo{BY: Deniz this is for you to address}

When the training data is incompletely observed, under the MAR model, it is natural for the modeler to instead choose a causal structure that maximizes the probability of the partially observed data
%\todo{BY: this is where we can insert the reason for KL bounds etc}
\begin{equation}    \label{eqn:modeler-objective}
    \that = \argmax_{\vtheta \in \mathcal{D}} \E_{\rvr|\rvr\neq 0}\left[ \E_{\rvx_o|\rvr;\vtheta_p}\!\left[ \log \P_{\rvx_o;\vtheta}(\vx_o)\!\mid\! \rvr = \vr\right] \right].
\end{equation}
%This objective takes the equivalent and more useful form of
%\begin{align}
%\that &= \argmax_{\vtheta} \E_{\P_{\rvx;\vtheta_p}} \left[ %\sum_{\vr\neq 0} \P_{\rvr|\rvx,\rvr\neq 0}(\vr) \log \P_{\rvx_o}%(\vx_o;\vtheta) \right] \notag\\
 %& = \argmax_{\vtheta} \E_{\P_{\rvx;\vtheta_p}} \left[ \sum_{\vr\neq %0} \frac{\P_{\rvr|\rvx}(\vr)}{1 - \P_{\rvr|\rvx}(0)} \log \P_{\rvx_o}%(\vx_o;\vtheta) \right]. \label{eqn:modeler-objective}
%\end{align}
When the missingness model is indeed MAR, this formulation has the property that it leads to the same $\that$ as in the full-data case. 
%\todo{clarify and give reference.. this can't even be true, because this doesn't have a unique solution in general. think claim is that maximizing this is equivalent to maximizing the likelihood from the fully observed distribution.}
%\todo{BY: this needs to be revised Alex}

\subsection{Objective of the Modeler and Goals of the Adversary} Equation~\ref{eqn:modeler-objective} is taken to be the objective of the modeler in our approach to AM. Although modelers may choose arbitrary objectives to learn their causal structures, we find that in practice (see Section~\ref{sec:exp}) using~\eqref{eqn:modeler-objective} as a proxy objective yields successful attacks.

The solution $\that$ of \eqref{eqn:modeler-objective} is a function of the missingness mechanism $\P_{\rvr|\rvx}$. The adversary's aim is to find an adversarial SCM $\P_{\rvx;\vtheta_\alpha}$ and design an adversarial missingness mechanism $\P_{\rvr|\rvx}$ satisfying the following properties.

\begin{enumerate}
\item \textbf{Adversarial Markovianity:} $\P_{\rvx;\vtheta_\alpha}$ is Markov relative to the adversarial graph $\mathcal{G}_\alpha$.

\item \textbf{$\beta$-indistinguishability:} To foil the auditor, we impose the condition that the adversarial and true distributions must be within distance $\beta$ in KL-divergence. 
 
 \item \textbf{Bounded missingness rate:} The expected number of missing features per sample is bounded to reduce the chance that the modeler \textit{a priori} rejects the training data set as too incomplete to reliably infer causal structures. 
 
\item \textbf{Attack success:} When \eqref{eqn:modeler-objective} is solved with $\P_{\rvr|\rvx}$, the distribution $\P_{\rvx;\that}$ learned by the modeler is Markov relative to $\mathcal{G}_\alpha$ and close in KL-divergence to $\P_{\rvx;\vtheta_\alpha}$.
\end{enumerate}
The adversary's objective is thus to find $\vtheta_\alpha$ and missingness mechanism $\P_{\rvr|\rvx}$ that solve
\begin{align}
\min_{\P_{\rvr|\rvx}, \vtheta_\alpha}\, & \text{D}_{\textrm{KL}}(\P_{\rvx;\vtheta_\alpha}\,\|\, \P_{\rvx;\that})  \label{eqn:adversarial-objective}\\ 
\text{subject to}\,\, & & \notag \\
& \text{D}_{\text{KL}}(\P_{\rvx;\vtheta_p}\,\|\, \P_{\rvx;\vtheta_\alpha}) \leq \beta,\notag \\
& \P_{\rvx;\vtheta_\alpha} \textrm{ is Markov relative to } \mathcal{G}_\alpha, \notag \\
& \E_{\rvx;\vtheta_p} \left[ \E_{\rvr|\rvx} \left[\frac{|\{j\,|\,\rvr_j=0\}|}{d}\right] \right] \leq \gamma. \notag
\end{align}
The attack success is measured by the value of the objective function and the Hamming distance between the returned SCM and $\mathcal{G}_\alpha$. 

This is an ambitious optimization problem, encoding multiple competing desiderata. It may not be possible to find an adversarial distribution that is $\beta$-indistinguishable from the true distribution while also being adversarially Markovian and satisfying an expected missingness rate under $\gamma$.

\subsection{A two stage approximation}

In the adversarial objective,~\eqref{eqn:adversarial-objective}, the adversary optimizes over the missingness mechanism and the adversarial SCM jointly, and $\beta$-indistinguishability is a hard constraint. To mitigate the difficulty of this joint optimization and hard constraint, we propose a two stage approximation. 

In the first stage, the adversary selects a target adversarial SCM $\P_{\rvx; \ta}$ that is Markov with respect to $\mathcal{G}_\alpha$ and minimizes the KL-divergence to the true SCM. In the second stage, the adversary finds a missingness mechanism that guides the modeler to learn $\ta$ and has a bounded missingness rate. Specifically, we propose to first solve
\begin{align}
	\ta=\argmin_{\vtheta \in \mathcal{D}_\alpha},  \text{D}_{\text{KL}}(\P_{\rvx;\vtheta_p}\,\|\, \P_{\rvx;\vtheta}) \label{eq:KLmin},
\end{align}
where $\mathcal{D}_\alpha\defeq\{\vtheta:\P_{\rvx;\vtheta} \textrm{ is Markov relative to } \mathcal{G}_\alpha\}$ denotes the set of feasible $\vtheta$. Next, we optimize the original objective with $\ta$ fixed, and relax the hard constraint using a Lagrange multiplier:
\begin{align}
	\min_{\P_{\rvr|\rvx}}\ \text{D}_{\textrm{KL}}(\P_{\rvx;\vtheta_\alpha}\,\|\, \P_{\rvx;\that}) + \lambda \E_{\rvx;\vtheta_p} \left[ \E_{\rvr|\rvx} \left[\frac{|\{j\,|\,\rvr_j=0\}|}{d}\right] \right]. \label{eqn:adversarial-objective2}
\end{align}
This two-stage approximation has the advantage of not requiring an a priori selection of $\beta$ and $\gamma$. Instead, the smallest possible $\beta$ is implicitly selected in the first stage, and by varying $\lambda$ the adversary can explore the trade-off between ensuring $\that$ is close to $\vtheta_\alpha$ and ensuring that the missingness mechanism has a small expected missingness rate.

%The optimal value of~\eqref{eqn:adversarial-objective2} is an upper bound and a solution to Eq. \ref{eqn:adversarial-objective2}, is not necessarily feasible for Eq. \ref{} (there might be $\ta$ with higher KL divergence but lower missing data). Nevertheless, it's a useful approximation in practise.

In Appendix~\ref{sxn:optimal_adversarial_scm_selection}, a characterization of the optimal adversarial SCM is given for an arbitrarily parameterized family of SCMs, assuming that the adversarial DAG is a subgraph of the true DAG. In the special case of linear Gaussian SCMs, this leads to a closed form solution for the optimal adversarial SCM.

\begin{theorem}[Optimal Adversarial SCM for linear Gaussian SCMs]
\label{thm:optimal_adversarial_linear_gaussian_SCM}
    Let $\P_{\rvx; \vtheta_p}$ be a mean-zero linear Gaussian SCM that is Markov with respect to $\mathcal{G}_p$, so $\rvx; \vtheta_p \sim \mathcal{N}(\bm{0}, \bm{\Sigma})$, and let $\mathcal{G}_\alpha$ be a subgraph of $\mathcal{G}_p.$ Denote the parents of $\rvx_j$ in $\mathcal{G}_\alpha$ by $\overline{\pa}_j$ and the parents of $\rvx_j$ in $\mathcal{G}_p$ by $\pa_j$. 
    
    The linear Gaussian SCM closest to $\P_{\rvx; \vtheta_p}$ in KL-divergence that is Markov with respect to $\mathcal{G}_\alpha$ is given by 
\[
 \mathbf{X} = \mB_\alpha^T \mathbf{X} + \vn,
 \]
 where $\vn \sim \mathcal{N}(\bm{0}, \mD)$ with
 \[
  \mD = \operatorname{Diag}\left(\left\{\bm{\Sigma}_{j,j} - \left \langle\bm{\Sigma}_{\overline{\pa}_j,j}, \left(\bm{\Sigma}_{\overline{\pa}_j, \overline{\pa}_j}\right)^{-1} \bm{\Sigma}_{\overline{\pa}_j,j}\right\rangle\right\}_{j=1}^d\right),
 \]
 and the $j$th column of $\mB$ is the vector 
 \[
 \vb_j = \mR_{\overline{\pa}_j}^T \left(\bm{\Sigma}_{\overline{\pa}_j, \overline{\pa}_j}\right)^{-1} \bm{\Sigma}_{\overline{\pa}_j,j},
 \]
where $\mR_{\overline{\pa}_j} \in \mathbb{R}^{|\overline{\pa}_j| \times d}$ is the restriction operator that satisfies $\mR_{\overline{\pa}_j} \vx = \vx_{\overline{\pa}_j}.$
\end{theorem}

This result is used to select adversarial SCMs in our experimental evaluations.

\section{Adversarial Missingness via Generalized Rejection Sampling}
\label{sxn:generalized_rejection_sampling}

Our first result establishes a general procedure for guiding modelers that optimize~\eqref{eqn:modeler-objective} to produce $\that = \vtheta_\alpha$, when the adversary has access to a $\beta$-indistinguishable adversarial SCM. The approach uses rejection sampling, so the bound on the missingness rate is implicitly determined by the relationship between $\P_{\rvx;\vtheta_\alpha}$ and $\P_{\rvx;\vtheta_p}$.

The intuition behind the approach is to employ a missingness mechanism that biases towards choosing the observation pattern so that the observed features are more probable under $\P_{\rvx_o}(\cdot; \vtheta_\alpha)$ than under $P_{\rvx_o}(\cdot; \vtheta_p).$ Specifically, let $\vr \in \{0,1\}^d$ be a fixed nonzero observation mask, then define the ratio of the two probabilities for the corresponding observed features as 
\[
\Lambda_\vr(\vx_o) := \frac{\p_{\rvx_o}(\vx_o; \vtheta_\alpha)}{\p_{\rvx_o}(\vx_o; \vtheta_p)}
\]
and take $\Lambda_\vr^\star = \max_{\vx_o} \Lambda_\vr(\vx_o)$ to be the largest value of this ratio; we assume that the adversarial SCM is chosen so that $\Lambda_\vr^\star$ is finite. Now define the probability that the adversary chooses $\rvr = \vr$, conditional on observing the sample $\vx$ from $\P_{\rvx;\vtheta_p}$, in terms of these quantities,
\begin{equation}\label{eqn:generalized_rejection_sampler}
\p_{\rvr|\rvx}(\vr|\vx) = \begin{cases}
\pi_{\vr} \frac{\Lambda_\vr(\vx_o)}{\Lambda_\vr^\star} & \text{ if } \vr \neq 0 \\
1 - \sum_{\vr^\prime \neq 0} \pi_{\vr^\prime} \frac{\Lambda_{\vr^\prime}(\vx_{o^\prime})}{\Lambda_{\vr^\prime}^\star} & \text{ if } \vr = 0
\end{cases}.
\end{equation}
Here, the indices $o^\prime$ are defined with respect to $\vr^\prime$ and the weights $\pi_{\vr}$ satisfy $0 \leq \pi_{\vr} \leq 1$ for all $\vr \neq 0$. 

If the $\pi_{\vr}$ are selected so that the quantity defining the probability of $\rvr = 0$ conditional on $\rvx=\vx$ is nonnegative for all values of $\vx$, then the proposed missingness mechanism is a valid distribution. The choice $\pi_{\vr} = \frac{1}{2^d - 1}$, which assigns uniform weight to all nonzero observation patterns, is always valid, independent of the choice of the adversarial and true distributions; this is true because $\Lambda_{\vr}/\Lambda_{\vr}^\star \leq 1$ always, for all non-zero observation patterns $\vr$.

It is worth noting that for this mechanism, the MAR assumption fails only at $\vr = 0$, as otherwise $\rvr$ depends only on the observed features $\vx_o$, so $\rvx_m \perp \rvr = \vr \,|\, \rvx_o$. 

Our first observation is that this generalized rejection sampling approach ensures that the partially observed features from $\P_{\rvx;\vtheta_p}$ look as though they were sampled from the adversarial distribution.

\begin{lemma}[Generalized Rejection Sampling]\label{lem:generalized_rejection_sampling}
	The distribution over the observed features induced from $\P_{\rvx; \vtheta_p}$ by the missingness mechanism defined in~\eqref{eqn:generalized_rejection_sampler} satisfies
 \[\P_{\rvx_o \mid \rvr}(\cdot\,| \vr; \vtheta_p)=\P_{\rvx_o}(\cdot \,;\vtheta_\alpha)\]
 for all $\vr\neq 0$.
\end{lemma}

When the missingness mechanism is such that the partially observed features for any observation pattern are distributed as though they were drawn from the adversarial distribution, the adversary is able to manipulate the modeler into thinking the observed data comes from the adversarial distribution.

\begin{theorem}[Global Optimality of the Adversarial SCM]\label{thm:rejection_sampling_global_maximizer}
When the adversarial missingness mechanism $\P_{\rvr|\rvx}$ satisfies the condition
\[\P_{\rvx_o \mid \rvr}(\cdot\,| \vr; \vtheta_p)=\P_{\rvx_o}(\cdot \,;\vtheta_\alpha)\]
for all $\vr\neq 0$, it is the case that $\vtheta_\alpha$ is a global maximizer of the modeler's objective (\eqref{eqn:modeler-objective}).
\end{theorem}

It follows immediately that the adversarial model is a global maximizer of the modeler's objection~\eqref{eqn:modeler-objective}. 

\begin{corollary}\label{cor:attack_success_generalized_rejection_sampling}
When the adversarial missingness distribution is constructed using the generalized rejection sampling of~\eqref{eqn:generalized_rejection_sampler}, $\vtheta_\alpha$ is a global maximizer of the modeler's objective (\eqref{eqn:modeler-objective}).
\end{corollary}

This result shows that generalized rejection sampling achieves several of the goals of the adversary stipulated in Section~\ref{sxn:formulation}. Specifically, if one assumes that the adversary has chosen an adversarial distribution that is $\beta$-indistinguishable and satisfies adversarial Markovianity, then Corollary~\ref{cor:attack_success_generalized_rejection_sampling} states that the attack succeeds in the sense that the adversarial model is a maximizer of the modeler's objective. As the modeler's objective is nonconvex and may have multiple global optima, this seems likely to be the strongest type of result one can obtain on attack success without restricting the class of SCMs under consideration.

A bound on the missingness rate for the generalized rejection sampling missingness mechanism can be given. Recall that for the missingness mechanism in~\eqref{eqn:generalized_rejection_sampler} to be well-defined, the weights $\pi_\vr$ must be selected to ensure that the probability of sampling $\rvr = 0$ given $\rvx = \vx$ is nonnegative for any $\vx$. The choice of weights also affects the bound on the missingness rate.

\begin{lemma}\label{lem:generalized_rejection_sampling_missingness_bound}
Let $\ell_{\vr} = |\{j \mid \vr_j = 0\}|$ denote the amount of features missing in pattern $\vr$. When generalized rejection sampling is used, the expected missingness rate is given by
\[
\E_{\rvr}\left[\frac{|\{j\,|\,\rvr_j=0\}|}{d}\right] = 1 - \sum_{\vr \neq 0} \frac{\pi_\vr}{\Lambda_\vr^\star} \left(1 - \frac{\ell_{\vr}}{d} \right)
\].
\end{lemma}

Lemma~\ref{lem:generalized_rejection_sampling_missingness_bound} shows that the choice of $\pi_{\vr}$ has an important effect on the missingness rate. Specifically, it establishes the importance of employing large weights $\pi_{\vr}$ in order to reduce the expected amount of missing data. It is difficult to select admissible and large $\pi_{\vr}$, as the weights must be chosen so that the probability of sampling $\rvr = 0$ conditional on \emph{any} sample $\rvx = \vx$ is a valid probability. 

As noted earlier, the choice $\pi_{\vr} = (2^d - 1)^{-1}$ is \emph{always} admissible. However, in cases where the adversarial SCM is close to the true SCM, one can find missingness mechanisms with significantly tighter bounds on their missingness rate by utilizing \emph{localized generalized rejection sampling.}

\subsection{Local Generalized Rejection Sampling}



Let $\mathcal{V} \subseteq \{1, \ldots, d\}$ denote a subset of the variables, and $\overline{\mathcal{V}}$ denote the complement. Localized generalized rejection sampling on the variables $\mathcal{V}$ is a missingness mechanism that masks only variables in $\mathcal{V}$, using probabilities depending only on the value of $\rvx_{\mathcal{V}}$, given by

\begin{equation}\label{eqn:localized_generalized_rejection_sampling}
\P_{\rvr|\rvx}(\vr|\vx) = \begin{cases}
\frac{1}{2^{|\mathcal{V}|}-1} \frac{\Lambda(\vx_{\mathcal{V}})}{\Lambda} & \text{ if } \vr_{\overline{\mathcal{V}}}=1 \text{ and } \vr_{\mathcal{V}} \neq 0 \\
1 - \frac{\Lambda(\vx_{\mathcal{V}})}{\Lambda} & \text{ if } \vr_{\overline{\mathcal{V}}}=1 \text{ and } \vr_{\mathcal{V}} = 0 \\
0 & \text{ otherwise}
\end{cases}.
\end{equation}
Here, $\Lambda(\vx_{\mathcal{V}}) = \frac{\p_{\rvx_{\mathcal{V}};\vtheta_\alpha}(\vx_{\mathcal{V}})}{\p_{\rvx_{\mathcal{V}};\vtheta_p}(\vx_{\mathcal{V}})} $ and  $\Lambda = \max_{\vx_{\mathcal{V}}} \Lambda(\vx_{\mathcal{V}}).$ Note that the observation patterns that select all variables in $\overline{\mathcal{V}}$ and at least one variable in $\mathcal{V}$ are equiprobable. The missingness rate of this approach is at most $\tfrac{|\mathcal{V}|}{d}$, which is significantly better than the worst-case $O(1)$ missingness rate of generalized localized sampling. Lemma~\ref{lem:localized_generalized_rejection_sampling_missingness_bound} in the Appendix establishes a tighter bound on the missingness rate that depends on the ratio $\Lambda$.

When the conditional distributions of the variables in $\overline{\mathcal{V}}$ given the variables in $\mathcal{V}$ is identical in the adversarial and true SCMs, localized generalized rejection sampling ensures that the partially observed features from $\P_{\rvx;\vtheta_p}$ look as though they were sampled from the adversarial distribution.

\begin{lemma}[Localized Generalized Rejection Sampling]
\label{lem:localized_generalized_rejection_sampling}
Let $\mathcal{V} \subset \{1, \ldots, d\}$ be a subset of the variables. If it is the case that the adversarial distribution preserves the dependence of $\overline{V}$ on $\mathcal{V}$, that is,
\[
\P_{\rvx_{\overline{\mathcal{V}}} \mid \rvx_{\mathcal{V}}}( \cdot \mid  \cdot\,; \vtheta_\alpha) = \P_{\rvx_{\overline{\mathcal{V}}} \mid \rvx_{\mathcal{V}}}(\cdot \mid \cdot\, ; \vtheta_p),
\] and the adversary uses the missingness mechanism defined  in~\eqref{eqn:localized_generalized_rejection_sampling}, then
\begin{equation}
\label{eqn:matched_conditional_distribution}
\P_{\rvx_o\mid \rvr}(\cdot\,\mid \vr; \vtheta_p) = \P_{\rvx_o}(\cdot\,; \vtheta_\alpha)
\end{equation}
for all $\vr$ such that $\P_{\rvr}(\vr) \neq 0$.
\end{lemma}

This result implies that when the matching condition~\eqref{eqn:matched_conditional_distribution} holds, the adversary can attain their goal of causing $\vtheta_\alpha$ to be a global maximizer of the modeler's objective.

\begin{corollary}\label{cor:attack_success_localized_generalized_rejection_sampling}
If it is the case that the adversarial distribution satisfies
\[
\P_{\rvx_{\overline{\mathcal{V}}} \mid \rvx_{\mathcal{V}}}( \cdot \mid  \cdot\,; \vtheta_\alpha) = \P_{\rvx_{\overline{\mathcal{V}}} \mid \rvx_{\mathcal{V}}}(\cdot \mid \cdot\, ; \vtheta_p)
\]
and the adversary uses localized generalized rejection sampling (\eqref{eqn:localized_generalized_rejection_sampling}), then $\vtheta_\alpha$ is a global maximizer of the objective of the modeler (\eqref{eqn:modeler-objective}).
\end{corollary}

As an example application, consider the case in which $\mathcal{G}_\alpha$ is obtained from $\mathcal{G}$ by deleting some number of incoming edges to a node $s$ and the adversarial SCM is constructed by preserving the functional relationships between $j$ and its parents whenever $j \neq s$ and imposing some new functional relationship between $s$ and its reduced set of parents. Then it is the case that~\eqref{eqn:matched_conditional_distribution} holds, so that the adversarial distribution is a global maximizer of the modeler's objective when localized generalized rejection sampling is used with $\mathcal{V} = \{s\} \cup \pa_s$.

\begin{corollary}[Local Edge Deletion]
\label{cor:local_edge_deletion}
Distinguish between the parents of variable $j$ in $\mathcal{G}$ and in $\mathcal{G}_\alpha$ by denoting the former with $\pa_j$ and the latter with $\overline{\pa}_j$. Select a $\mathcal{G}_\alpha$ such that $\overline{\pa}_j$ = $\overline \pa_j$ for all $j \neq s$ and $\overline{pa}_s \subseteq \pa_s$. If the adversarial distribution satisfies
\[
\P_{\rvx_j\mid\rvx_{\pa_j}}(\cdot\mid\cdot\,;\vtheta_p) = \P_{\rvx_j\mid\rvx_{\pa_j}}(\cdot\mid\cdot\,;\vtheta_\alpha) \text{ when $j \neq s$},
\]
then~\eqref{eqn:matched_conditional_distribution} holds and it follows that when the adversary uses localized generalized rejection sampling (\eqref{eqn:localized_generalized_rejection_sampling}) with $\mathcal{V} = \{s\} \cup \pa_s$, then $\vtheta_\alpha$ is a global maximizer of the objective of the modeler.
\end{corollary}


%Section~\ref{sxn:gaussian_proofs} of the Appendix provides approaches for adversarial missingness attacks, along with analysis, specifically for the case of linear Gaussian SEMs. In particular, in this case given an adversarial DAG $\mathcal{G}_\alpha$, one can determine exactly for which $\beta$ there exist $\beta$-indistinguishable adversarial SCMs that are Markov with respect to $\mathcal{G}_\alpha$. 
\section{Learned Adversarial Missingness Mechanisms (LAMM)}
\label{sxn:neural_approach}

The generalized rejection sampling approaches can be applied to finite training data sets, but offer little control of the missingness rate and their optimality guarantees hold when the modeler can evaluate the expectations involved in its objective. It is attractive to consider approaches that tailor the adversarial missingness mechanism specifically to the finite training data set at hand, and that explicitly encourage the missingness rate to be low.

With finite data, the expectations in~\eqref{eqn:modeler-objective} must be replaced with empirical averages. Moreover, even for SCMs parameterized with exponential family distributions, the objective is non-concave due to the presence of missing data, which leads practitioners to use the Expectation Maximization (EM) algorithm to learn the parameters. In this setting, the adversary's goal is to select a missingness distribution such that EM converges to the adversarial parameter $\ta$.

To that end, we propose to parameterize the missingness distribution with a neural network. Let $\midx$ denote the variables the adversary chooses for local masking and $y(\vx_\midx,\vphi)=\text{softmax}((f^{L}\circ \dots \circ f^{1})(\vx_\midx))$ be an $L$-hidden layer neural network with $2^{|\midx|}$ output units; here
$\vphi$ are the parameters of the network. Each output unit returns the probability of one of the observation patterns $\vr_{\mathcal{V}}$. Let $\delta:\{0,1\}^{|\midx|}\rightarrow \{0,1,\dots,2^{|\midx|}-1\}$ denote the function that maps the observed mask pattern to the corresponding output neuron. Then the missingness distribution is parameterized as follows:
\begin{equation}
\P_{\rvr|\rvx}(\vr|\vx,\vphi)= 
\begin{cases}
    y(\vx_\midx,\vphi)_{\delta(r_{\midx})},&\text{if } \vr_{\overline{\midx}}=1\\
0,              &\text{otherwise}
\end{cases}
\end{equation}

Our goal is to optimize the adversary's objective, \eqref{eqn:adversarial-objective2} by choosing $\vphi$ appropriately. Recall that the modeler, given partially observed data sampled according to the adversary's missingness mechanism, chooses the parameter $\that$ in~\eqref{eqn:adversarial-objective2} by solving its own objective~\eqref{eqn:modeler-objective}. In order to learn an optimal $\vphi$ to parametrize the adversary's missingness mechanism, we model the dependence of $\that$ on $\vphi$ in a differentiable manner.

The EM algorithm is the canonical approach to finding a minimizing $\that$ for~\eqref{eqn:modeler-objective} given a single sampled realization of the missingness mechanism, but because of the sampling process, its output $\that$ is not differentiable with respect to $\vphi$. Instead of sampling from the missingness mechanism, we take the expectation with respect to it; this results in a differentiable objective. We call this formulation the Weighted EM (WEM) algorithm.

Denote the missingness weights by
\[
\omega_{i,r}(\vphi)=\frac{\P_{\rvr \mid \rvx} (\vr \mid \vx^{(i)} ; \bm{\phi})}{\sum_{\vr^\prime \neq 0} \P_{\rvr \mid \rvx } (\rv^\prime\mid \vx^{(i)}; \bm{\phi})},
\]
where $\data = \{\vx^{(i)}\}_{i=1}^N$ is the fully observed training data. Given the parameters $\vtheta^{t-1}$ from the previous step, the expectation step of WEM is the calculation of
\begin{multline}
	Q(\vtheta, \vtheta^{t-1},\bm{\phi}) = \\
	\sum_{i=1}^N \sum_{\vr\neq 0}\omega_{i,r}(\vphi)
	\E_{\rvx;\vtheta^{t-1}}\left[\log \P_{\rvx}(\rvx; \vtheta) \mid \rvx_{o}=\vx_{o}^{(i)}\right] \label{eqn:expectation_step_of_WEM}
\end{multline}
When $N$ is large, by the law of large numbers the expectation step of EM is close to the expectation step of WEM. 
%Because 
%A natural way to solve~\eqref{eqn:modeler_objective_2}, given finite training data, is to use a EM algorithm. 

%Given this observation, we propose a heuristic that learns an adversarial missingness mechanism that causes the weighted EM algorithm to converge to the desired adversarial SCM. We find empirically that this approach also allows the adversary to succeed against other modern approaches to learning SCMs. 


\begin{comment}
{\bf Outline:
- Recall modeler thinks we are in MAR setting so reasonable approach is to use EM because "consistent" (meaning?) in infinite data limit. Give reference for this claim.
- Find empirically this likelihood-based approach also allows adversary to succeed against other modern approaches to learning DAGs
- provide a general heuristic for matching adversarial distribution via learning a neurally parameterized missingness model: input is adversarial distribution and data from true distribution.
- To be robust to modeler choices, use multiple starting points and use stopping criterion employed}

\end{comment}

%$ with a parameter $\bm{\phi}$ to be learned, and use the weights
The maximization step of WEM does not employ a DAG constraint, and is given by
\begin{equation}\label{eq:wem}
	\vtheta^t = \argmax_{\vtheta} Q(\vtheta, \vtheta^{t-1},\bm{\phi}).
\end{equation}

The WEM Algorithm, which repeats WEM expectation and maximization steps until convergence of the parameters $\vtheta^t$, is described in Algorithm~\ref{alg:wem}. It utilizes a likelihood-based stopping criterion. Specifically, an empirical approximation of the modeler's objective function in ~\eqref{eqn:modeler-objective} is used to measure the probability of the observed data; again, the expectation over the missingness mechanism is explicitly computed:
\begin{equation}
\label{eqn:empirical_likelihood}
J(\vtheta,\vphi) = \sum_{i=1}^N \sum_{r\neq 0} \omega_{i,r}(\vphi) \log \P_{\rvx_o}(\vx^{(i)}_o;\vtheta)
\end{equation}

\begin{algorithm}[tb]
	\caption{WEM Algorithm. Solves the weighted EM problem corresponding to a given missingness mechanism, using a likelihood-based stopping criterion. Both the likelihood $J(\vtheta,\vphi)$ (\eqref{eqn:empirical_likelihood}) and the expectation $Q(\vtheta, \vtheta^{t-1},\bm{\phi})$ (\eqref{eqn:expectation_step_of_WEM}) use the fully observed samples, $\data$. This dependence is omitted from the notation for brevity.}
	\label{alg:wem}
	
	\begin{algorithmic}
		\STATE {\bfseries Input: $\vphi, \vtheta^{0}, \epsilon, \data$ }
		%		\State $\tat{0}\leftarrow\tr$
		\STATE $t\leftarrow 1$
		\WHILE{$J(\vtheta^{(t)},\bm{\phi})-J(\vtheta^{(t-1)},\bm{\phi})\geq \epsilon |J(\vtheta^{(t-1)},\bm{\phi})|$} 
		\STATE $\vtheta^{t}= \argmax_{\vtheta} Q(\vtheta, \vtheta^{t-1},\bm{\phi}) $
		\STATE $t\leftarrow t+1$
		\ENDWHILE
		\STATE $\ttil \leftarrow \vtheta^{t-1}$
		\STATE {\bfseries Output: $\ttil$} 
	\end{algorithmic}
\end{algorithm}

Given that the modeler's procedure for optimizing its objective to learn $\that$ is captured by the WEM algorithm, the adversary's goal is to make WEM converge to $\ta$ from an arbitrary starting point $\vtheta^{0}$. Denote the corresponding output of Algorithm~\ref{alg:wem} by $\text{WEM}(\vphi,\vtheta^{0},\epsilon,\data)$. The adversary solves the following problem using gradient-based optimization:
\begin{align}\label{eq:wem2}
		\min_{\vphi } & \quad \text{D}_{\text{KL}}(\P_{\rvx;\vtheta_\alpha} \| \P_{\rvx;\ttil})\,\,+ \\
  & \frac{\lambda}{N}\sum_{i=1}^N \E_{\rvr|\rvx;\vphi} \left[\frac{|\{j\,|\,\rvr_j=0\}|}{d}\,\Big\lvert\, \rvx=\vx^{(i)}\right] \notag \\
		&\kern-2em \text{where } \ttil =\text{WEM}(\vphi,\vtheta^{0},\epsilon,\data). \notag
\end{align}
This formulation accounts for the adversary's desire to bound the expected missingness rate in~\eqref{eqn:adversarial-objective2}. The constraint on the expected missingness rate is converted to a regularization term with Lagrange multiplier $\lambda$ where the expected missingness rate is estimated empirically. In general, solving this optimization problem requires the WEM algorithm to be started from scratch in each training epoch using the updated weights. For exponential family distributions, the maximization step of WEM (\eqref{eq:wem}) admits a simple form. Details are given in Appendix~\ref{app:wem}. 

In practice, the modeler's initialization scheme is unknown, and the adversary could overfit to a particular initialization when solving~\eqref{eq:wem2}. To mitigate this, $\vphi$ is selected to guide multiple random initializations to $\ta$. The proposed method of learning a missingness distribution is described in Algorithm~\ref{alg:nn}.

\begin{algorithm}[tb]
	\caption{LAMM Algorithm. Learns the adversarial missingness mechanism by directing weighted EM to converge on a desired parameter. The subroutine WEM is described in Algorithm~\ref{alg:wem}. $\ell (\ttil_k, \ta,\vphi,\lambda)$ denotes the objective function given in \eqref{eq:wem2}}.
	\label{alg:nn}
	
	\begin{algorithmic}
		\STATE {\bfseries Input: $\vtheta_\alpha, \epsilon, K, \data$, $\lambda$}
		%		\State $\tat{0}\leftarrow\tr$
		\STATE $\bm{\phi} \leftarrow \text{Initialize}$
		\STATE $\vtheta^{0}_k\leftarrow \text{Initialize } \ k=1,\dots,K$ 
		\WHILE{$\bm{\phi}$ not converged}
		\STATE  \COMMENT{Using $K$ starting points for robustness}
		\FOR{\texttt{$k=1,\dots,K$}}
		\STATE $\tilde{\vtheta}_k \leftarrow \text{WEM}(\vphi, \vtheta^{0}_k, \epsilon, \data)$ \COMMENT{WEM Algorithm}
		\ENDFOR
		\STATE $\bm{\phi} \leftarrow \bm{\phi}- \frac{\eta }{K}\sum_{k=1}^K\nabla_{\bm{\phi}} (\ell (\ttil_k, \ta,\vphi,\lambda))$
		\ENDWHILE
		\STATE {\bfseries Output: $\bm{\phi}$} 
	\end{algorithmic}
\end{algorithm}

%Although, the longer the convergence of WEM takes the longer the backprogate needs to track, it didn't caused a problem in practise.

The LAMM formulation is flexible and, when more is known about the subroutine the modeler is using to learn $\that$, one can replace WEM with an appropriate differentiable subroutine. We leave it as future work to investigate such alternative proxies for the modeler's structure learning objective.

\section{Experiments}\label{sec:exp}

The experimental setup has three components corresponding to parts of the adversarial missingness threat model shown in Figure~\ref{fig:overall}: the underlying true SCM ($\tr$); the causal discovery algorithm employed by the modeler; and the adversary's choice of the adversarial DAG, adversarial SCM, and missingness mechanism ($\ga,\ta,\prx$).

\input{table.tex}

\textbf{The true SCM.} For the true SCMs we have used linear Gaussian SCMS with equal noise variance, as they are a popular choice (e.g. \cite{missdag, notears,golem}). Two of the experiments use simulated data, and one utilizes the commonly used Sachs dataset~\cite{sachs}. In each experiment, a single edge was targeted for deletion via adversarial missingness. Salient characteristics of the experiments are provided in Table~\ref{tab:experiment_stats}. 

\textbf{Modeler's Casual Structure Learning Algorithm.} For the modeler's causal structure learning algorithms we have employed methods developed for learning in the presence of missing data, namely the MissDAG \cite{missdag} (denoted as MissDAG (NT)), a score based method, and MissPC~\cite{misspc}, a constraint-based method. We have also compared with approaches that use mean imputation followed by structure learning algorithms that require fully observed data; namely, we have utilized mean imputation followed by the NOTEARS~\cite{notears} and PC algorithms. MissDAG is sensitive to the initialization of the parameters,  so we initialized the covariance matrices using five different schemes: Empirical Diagonal (``Emp. Diag.''), identity matrix (``Ident.''), the ground truth covariance matrix (``True''), a scaled random covariance matrix (``Random(*)'') and a scaled inverse Wishart random matrix (``IW(*)''). For details refer to Appendix \ref{app:init}.

\textbf{Adversary's Choices}. In each experiment, we describe how $\ga$ and the adversarial SCM are selected. The adversarial missingness distribution $\prx$ (denoted as MNAR in the tables) is either a variation of generalized local rejection sampling (\eqref{eqn:localized_generalized_rejection_sampling}) or selected via the \namenn algorithm (Algorithm \ref{alg:nn}). To test the relative advantages of our adversarial missingness mechanisms, we also employ missingness distributions that drop an equal amount of data completely at random. These distributions are denoted MCAR in the tables. To match the amount of missing data and the marginal distribution over the observation masks, the MCAR distributions are taken to be the marginal distribution of $\rvr$ given the MNAR missingness distribution $\P_{\rvr \mid \rvx}$ , i.e., $\P_{\rvr}(\vr) = \E_{\rvx; \vtheta_p}[ \P_{\rvr \mid \rvx}(\vr)]$. 

%Given a dataset $\data$, and a missing data distribution, $\P_{\rvr|\rvx}(\vr|\vx,\vphi)$, we first create a partially observed dataset by sampling the masks as $\vr^{(i)} \mid \vx^{(i)}\sim $ and 

\textbf{Performance Metrics} To measure the performance of the adversarial missingness attacks, we first sample data from the true SCM and generate missing data masks ${\vr^{(i)} \mid \vx^{(i)}\sim \prx(\cdot\,;\,\vx^{(i)})}$ according to the relevant missingness mechanism, and generate masked data sets $\{\hat{\vx}^{(i)}\}_{i=1}^N$ where $\hat{\vx}^{(i)}$ has observed values in $\vr^{(i)}$ and NaNs to denote the missing entries. Given the partially observed data, we employ the relevant causal structure learning algorithm to estimate an SCM with corresponding DAG $\mathcal{\hat{G}}$. We report the Hamming distance (HD), the number of edge differences, between $\mathcal{\hat{G}}$ and $\mathcal{G}_p$. If $\mathcal{\hat{G}}$ is a partial DAG, for each edge in the true graph, partial DAG has to contain the corresponding undirected edge. The adversarial attack is deemed successful if the edge targeted for deletion is not present in $\mathcal{\hat{G}}$. To account for the randomness in the missing data masks, this process is repeated multiple times and the average success rate and HD are reported.


All experiments involving a neural network employ a 2-hidden layer network with ReLu activation and 100 units per layer; see Appendix \ref{app:nn} for implementation details. 

\subsection{Simulation Experiments}

In our two simulation experiments, we have used a Gaussian SCM,
\begin{equation}
	\rvx = \mB^T \rvx + \vn,
	\label{eqn:gscm}
\end{equation}
where $\vn$ comprises independent Gaussian noise distributed as $\mathcal{N}(0, \mI)$.
%and $\mD = \text{diag}(\sigma_1^2, \ldots, \sigma_d^2)$ is a diagonal matrix.

In both experiments the adversarial goal is to remove a single edge. Let $(p,c)$ denote the parent and the child nodes corresponding to the removed edge. The removed edge $\wa_{i,j}=0$ is set to zero unless otherwise stated. Following Theorem~\ref{thm:optimal_adversarial_linear_gaussian_SCM}, the parameters $\mB^\alpha$ are kept the same as those of the true SCM except at the removed edge i.e. $\wa_{i,j}=\mB_{i,j}$ for all $(i,j)\neq (p,c)$ and $\sa_j=1$ for all $j\neq c$. We take $\sa_c=\sigma$, which is not optimal in terms of the KL-divergence between the adversarial SCM and the true SCM, but is consistent with the modeler's assumptions of equal variance.

\subsubsection{Gaussian SCM, I}

%The graph is displayed in Fig. xx.

We designed this experiment as a feasibility check of the LAMM approach with the local masking. The graph has three nodes, and nodes 2 and 3 have incoming edges from node 1 (See Appendix \ref{app:scm1}). These edges have magnitudes $0.8$ and $0.9$, both of which are above the minimum threshold set in~\cite{notears} to eliminate spurious edges. This $\mB$ results in a Pearson correlation of roughly 0.6 between $\rvx_1$ and $\rvx_2$, which makes localized generalized rejection sampling feasible (as the maximum of the density ratio is kept reasonable) but non-trivial. 

The adversarial goal is to remove the edge from 1 to 2 i.e. $(p,c)=(1,2)$ and the adversary employs LAMM with $\lambda=1e-2$. Following Lemma~\ref{lem:localized_generalized_rejection_sampling}, only nodes 1 and 2 are masked, so $\midx=\{1,2\}$. See Table \ref{tab:scm1}) for the experimental results. The trained missingness mechanism masks 40\% of the entries in the target two columns on average; the overall percentage of the training data masked is 27\%. LAMM ensures that the modeler converges to $\ga$ in all modeler configurations including when the modeler uses PC-based causal structure learning algorithms. These algorithms are very different from the EM-based algorithms that LAMM was designed to target. This experiment also suggests that the missingness mask must be selected on a per observation basis, as the MCAR missingness distribution never achieves the adversarial goal.

\subsubsection{Gaussian SCM, II}

This experiment is designed to gauge the effectiveness of the localized rejection attack Lemma~\ref{lem:localized_generalized_rejection_sampling}. We slighlty modified the equation for practical purposes (as described in Appendix~\ref{app:scm2}).

The true SCM is a 6 node graph with 5 edges, and the adversary aims to remove a single edge. The edges weights are selected randomly between $[0.5,2]\cup[-2,-0.5]$ as in~\cite{notears}, except for the edge between nodes 2 and 3.  To ensure the acceptance probability is at a reasonable level, we selected a low weight for the target edge: $\mB_{2,3}=0.4$. The edge weights, $\mB$, are given in Appendix~\ref{app:scm2}. 

The weight of the target edge is set to 0.25 in $\wa$, i.e. $\wa_{2,3}=0.25$, to increase the acceptance probability and because the NT algorithm uses a weight threshold at 0.3, as suggested by the authors~\cite{notears}.

The adversary utilizes the local rejection sampling algorithm, and following Lemma~\ref{lem:localized_generalized_rejection_sampling}, masks only $\midx=\{2,3\}$. In 
this experiment, the accepted samples are fixed to be fully observed. This results in $70\%$ of the rows of the two target columns missing entirely. The results, given in Table 3, show that the adversary achieves its goal when the modeler uses the missDAG algorithm, but not when the modeler uses the PC algorithm. This perhaps because the PC algorithm's significance threshold is lower than that of the NT algorithm. Although $\wa_{2,3}$ could be lowered, this would increas the maximum of the density ratios and result in unacceptable levels of missing data. 

%Because the NT algorithm thresholds the entries of estimate B 0.3, it  
%\subsubsection{Sachs}
\input{table_I.tex}
\input{table_II.tex}
\subsection{Sachs Dataset}

We used observational data from \citeauthor{sachs} \cite{sachs} to test our methods in a challenging setting. The data set contains only $N=853$ samples from a system with 11 different variables, and the ground truth SCM has 17 edges. This data set has posed a challenge to causal discovery algorithms even in the fully observed case (\cite{golem},\cite{zhuCausalDiscoveryReinforcement2020}). For this reason, our adversarial goal is to remove a correct edge from the DAG estimated from the fully observed data. 

\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\columnwidth]{nt_est_sachs_dashed.png}
	\caption{NT estimated graph in the Sachs dataset and two connected components. Dashed orange edge denotes the adversarial target.}
	\label{fig:nt}
\end{figure}
The NT algorithm estimated a DAG with 12 HD to the ground truth DAG (Figure \ref{fig:nt}) and managed to capture the two connected components present in the true DAG. Our adversarial goal is to remove the correctly estimated edge from ``plc'' to ``pip2''. In our formulation the ``true graph'' $\gp$ is the one estimated by the NT algorithm from the fully observed data.

Since this is a real dataset, the true SCM parameters $\tr$ are unknown, so we used the empirical covariance matrix while selecting the adversarial parameter in a heuristic way\footnote{The mean vector is set to zero after subtracting the average values from each column, following the assumptions in NT.}. Removing the edge between ``plc'' to ``pip2'' makes ``plc'' an isolated node, so we set the covariance terms from ``plc'' to ``pip2'' and ``plc'' to ``pip3'' zero. This approach is heuristic, but we observed that the covariance matrix corresponding to the NT estimated $\mB$ didn't match the empirical covariance matrix accurately. It suggests Gaussian SCM model might be inadacute and using $\mB$ directly may lead to unwanted changes in the distribution.

The adversary uses \namenn with $\lambda=0$ and following Lemma~\ref{lem:localized_generalized_rejection_sampling} masks only $\midx=\{\text{``plc'',``pip2'',``pip3''}\}$. The missingness distribution learned masks $51.0\%$ of the three masked variables, which corresponds to a missingness rate of $13.9\%$ over all the variables (See loss function Appendix Figure \ref{fig:loss}). 

The results are displayed in Table \ref{tab:sachs}. For missDAG and NT after mean imputation, \namenn has a higher success rate with relatively less unintentional edges added. \namenn has its lowest success rate ($70\%$) against missDAG with the random initializations. We also observed for missPC, even MCAR missingness has a $100\%$ success rate. This suggests that the PC algorithm does not converge to the graph that NT estimates from the fully observed data.

\input{table_sachs.tex}


\section{Conclusion}

This work introduced the adversarial missingness model for influencing the learning of structural causal models from data. This adversarial model is appropriate in settings where attempts by the adversary to manipulate the values of the data can be detected, and the ubiquity of benignly missing data supports the use of adversarial missingness as a vector of attack. 

Generalized rejection sampling schemes were introduced and proven to achieve many of the desiderata of adversarial missingness, thereby establishing a strong proof of concept of the threat model. As a practical methodology for AM with finite training data sets, we provided a heuristic for learning adversarial missingness mechanisms, and demonstrated its performance using data drawn from synthetic and real SCMs.

Many aspects of the AM threat model remain to be explored, e.g.: (1) can one design algorithms that provably achieve the desiderata of AM in the finite data setting, (2) can one quantify the trade-offs between the desiderata of the adversary (e.g. the missingness rate and the attack success or the missing rate and the $\beta$-indistinguishability), and (3) how modelers defend against AM attacks? We expect that meaningful answers to these questions depend on the functional form of the SCMs under consideration, and are currently investigating these issues in the context of linear Gaussian SCMs.

%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
\begin{acks}
To Robert, for the bagels and explaining CMYK and color spaces.
\end{acks}

%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\bibliographystyle{ACM-Reference-Format}
\bibliography{paper-refs}

%%
%% If your work has an appendix, this is the place to put it.
\clearpage
\appendix
%\onecolumn

\section{Characterization and Selection of Optimal Adversarial SCMs}
\label{sxn:optimal_adversarial_scm_selection}

(Localized) generalized rejection sampling provides a methodology for conducting adversarial missingness attacks on arbitrarily parameterized SCMs, \emph{if} the target adversarial SCM is known \emph{a priori} to satisfy $\beta$-indistinguishability and to be Markovian with respect to the adversarial DAG $\mathcal{G}_\alpha$. Similarly, the LAMM heuristic provides a sample efficient methodology under the same assumptions.

However, given the true SCM in an arbitary parameterized family of SCMs, an arbitrary $\beta$, and an arbitary adversarial DAG $\mathcal{G}_\alpha$, it is nontrivial to even determine whether a $\beta$-indistinguishable SCM that is Markovian with respect to $\mathcal{G}_\alpha$ exists, much more to find one. In this section, we provide a general characterization of optimal adversarial SCMs when $\mathcal{G}_\alpha$ is a subgraph of $\mathcal{G}_p$---the SCMs closest to $\P_{\rvx; \vtheta_p}$ in KL-divergence while also being Markov with respect to $\mathcal{G}_\alpha$. In the case of linear Gaussian SCMs, these characterizations provide a practical approach to finding an optimal SCM.

The key observation to obtaining our characterization is that the KL-divergence between two distributions that are Markov with respect to the same DAG satisfies a convenient factorization.

\begin{lemma}
\label{lem:factorize_KL}
If $\P_{\rvx; \vtheta_1}$ and $\P_{\rvx; \vtheta_2}$ are SCMs that are Markovian with respect to the DAG $\mathcal{G}$, then 
\begin{multline*}
 \operatorname{D}_{\mathrm{KL}}\left( \P_{\rvx;\vtheta_1} \,\|\, \P_{\rvx; \vtheta_2} \right) = \\
 \sum_{j=1}^d \E_{\rvx_{\pa_j};\vtheta_1} \left[ \operatorname{D}_{\mathrm{KL}}\left( \P_{\rvx_j\mid \rvx_{\pa_j}; \vtheta_1} \,\|\, \P_{\rvx_j \mid \rvx_{\pa_j}; \vtheta_2} \right) \right].
\end{multline*}
\end{lemma}

\begin{proof}
    Write the causal factorizations of the pdfs of the two distributions with respect to $\mathcal{G}$ as
$$
\p(\vx; \vtheta_1) = \prod_{j=1}^d p(\vx_j\,|\,\vx_{\pa_j}; \vtheta_1) \quad \text{ and } \p(\vx; \vtheta_2) = \prod_{j=1}^d p(\vx_j\,|\,\vx_{\pa_j}; \vtheta_2),
$$
and observe that, as a consequence of these factorizations, the KL-divergence satisfies
\begin{align*}
    \operatorname{D}_{\mathrm{KL}}\left( \P_{\rvx;\vtheta_1} \,\|\, \P_{\rvx; \vtheta_2} \right) & = 
    \E_{\rvx; \vtheta_1} \left[ \ln\left( \frac{\p(\vx; \vtheta_1)}{\p(\vx; \vtheta_2)} \right) \right] \\
   &  \kern-5em = \E_{\rvx; \vtheta_1} \left[ \sum_{j=1}^d \ln\left( \frac{\p(\vx_j \mid \vx_{\pa_j}; \vtheta_1)}{\p(\vx_j \mid \vx_{\pa_j} ; \vtheta_2)} \right) \right] \\
    & \kern-5em = \sum_{j=1}^d \E_{\rvx_{\pa_j \cup \{j\}}; \vtheta_1} \left[ \ln\left( \frac{\p(\vx_j \mid \vx_{\pa_j}; \vtheta_1)}{\p(\vx_j \mid \vx_{\pa_j} ; \vtheta_2)} \right) \right] \\
    & \kern-5em = \sum_{j=1}^d \E_{\rvx_{\pa_j}; \vtheta_1} \left[ \E_{\rvx_j \mid \rvx_{\pa_j}; \vtheta_1} \left[  \ln \left( \frac{\p(\vx_j \mid \vz; \vtheta_1)}{\p(\vx_j \mid \vz ; \vtheta_2)} \right) \,\Big\lvert\, \rvx_{\pa_j} = \vz \right] \right] \\
    & \kern-5em = \sum_{j=1}^d \E_{\rvx_{\pa_j}; \vtheta_1} \left[ \operatorname{D}_{\mathrm{KL}}( \P_{\rvx_j\mid \rvx_{\pa_j}; \vtheta_1} \,\|\, \P_{\rvx_j \mid \rvx_{\pa_j}; \vtheta_2} )\right].
\end{align*}
The third equation holds because the structural equation for $\rvx_j$ involves only the variables $\rvx_j$ and $\rvx_{\pa_j}$, and the following equation uses the tower property of conditional expectation.
\end{proof}

The preceding result suggests that when the adversarial DAG is a subgraph of $\mathcal{G}_p$, then the adversarial SCM that minimizes the KL-divergence from the true SCM will change a minimal number of structural equations: in particular, when the parents of $\rvx_j$ are the same in both graphs, using the same structural equation for $\rvx_j$ ensures that
\[
\E_{\rvx_{\pa_j};\vtheta_1} \left[ \operatorname{D}_{\mathrm{KL}}\left( \P_{\rvx_j\mid \rvx_{\pa_j}; \vtheta_1} \,\|\, \P_{\rvx_j \mid \rvx_{\pa_j}; \vtheta_2} \right) \right]= 0.
\]
This claim is a specific instance of a more general result characterizing the adversarial SCM that minimizes the KL-divergence from the true SCM.

\begin{corollary}
    \label{cor:adversarial_optimality_condition}
	Suppose $\mathcal{G}_\alpha$ is a subgraph of $\mathcal{G}_p$. If $\P_{\rvx; \vtheta_\alpha}$ is Markov relative to $\mathcal{G}_\alpha$ and satisfies
 \begin{multline*}
 \E_{\rvx_{\pa_j};\vtheta_p} \left[ \operatorname{D}_{\mathrm{KL}}( \P_{\rvx_j \mid \rvx_{\pa_j};\vtheta_p}  \,\|\, \P_{\rvx_j \mid \rvx_{\pa_j}; \vtheta_\alpha}) \right] \leq \\
  \E_{\rvx_{\pa_j};\vtheta_p} \left[ \operatorname{D}_{\mathrm{KL}}( \P_{\rvx_j \mid \rvx_{\pa_j};\vtheta_p}  \,\|\, \P_{\rvx_j \mid \rvx_{\pa_j}; \vtheta}) \right]
 \end{multline*}
 for all $\P_{\rvx; \vtheta}$ that are Markov relative to $\mathcal{G}_\alpha$, for all $j=1,\dots,d$, and for all values of $\rvx_{\pa_j}$, then $\vtheta_\alpha$ is a solution to 
 \[
 \argmin_{\vtheta\,:\, \P_{\rvx; \vtheta} \in \mathcal{D}} \operatorname{D}_{\mathrm{KL}}( \P_{\rvx ;\vtheta_p}  \,\|\, \P_{\rvx ; \vtheta}),
 \]
 where $\mathcal{D}$ denotes the set of SCMs that are Markov with respect to $\mathcal{G}_\alpha$
\end{corollary}


\begin{proof}
 Because $\mathcal{G}_\alpha$ is a subgraph of $\mathcal{G}_p$, any SCM that is Markov relative to $\mathcal{G}_\alpha$ is Markov relative to $\mathcal{G}_p$. In particular,  Lemma~\ref{lem:factorize_KL} applies and gives that
\[
\operatorname{D}_{\mathrm{KL}}( \P_{\rvx ;\vtheta_p}  \,\|\, \P_{\rvx ; \vtheta_\alpha}) \leq \operatorname{D}_{\mathrm{KL}}( \P_{\rvx ;\vtheta_p}  \,\|\, \P_{\rvx ; \vtheta}).
\]
\end{proof}


\begin{comment}
Recall that in linear Gaussian SCMs, each $\rvx_i$ is a linear function of its parents and the exogenous noise, which is normally distributed. More precisely, $\rvx$ satisfies the autoregressive relation
\begin{equation}
\rvx = \mW^T \rvx + \vn,
\label{eqn:gscm}
\end{equation}
where $\vn$ comprises independent mean-zero Gaussian noise distributed as $\mathcal{N}(0, \mD)$ and $\mD = \text{diag}(\sigma_1^2, \ldots, \sigma_d^2)$ is a diagonal matrix. The locations of the nonzeros in each row of the autoregression matrix $\mW$ indicate the parents of the corresponding variable. The matrix $\bm{\Sigma} = (\mI - \mW)^{-T}\mD(\mI-\mW)^{-1}$ is the covariance matrix of $\rvx$. Let $\bm{\Theta} = \bm{\Sigma}^{-1}$ denote the concentration or precision matrix of $\rvx$; it is known that the sparsity pattern of $\bm{\Theta}$ captures the causal structure up to moralization\footnote{A DAG is moralized by adding an edge between any pair of non-adjacent vertices that share a child, then making the graph undirected.}. 

\begin{theorem}[\cite{loh2014high}]
\label{thm:gaussian_graph_structure}
Suppose $\rvx$ is generated from a linear Gaussian SCM (\eqref{eqn:gscm}). Then $\bm{\Theta}$ reflects the graph structure of the moralized DAG: i.e., for $j \neq k$, we have $\bm{\Theta}_{jk} = 0$ if and only if $(j,k)$ is not an edge in the moralized DAG.
\end{theorem}

The characterization given by this theorem leads directly to a classical algorithm for inferring the causal structure of linear Gaussian SCMs from data~\cite{loh2014high}: first use the sparsity pattern of the inverse covariance matrix to define a moralized DAG, then find the best-scoring DAG that is consistent with the moralized DAG. In several cases, including when $\mD$ is scalar, this algorithm recovers the true DAG. This algorithm works as well when $\rvx$ does not have zero mean.

In this section, we parameterize linear Gaussian SCMs in terms of their means and inverse covariance matrices, so that $\P_{\rvx; \vtheta} = \mathcal{N}(\bm{\mu}, \bm{\Sigma})$, where $\bm{\Sigma} = \vtheta^{-1}$. Since the adversary has knowledge of the true SCM, and in particular the true mean $\bm{\mu}$, all potential adversarial SCMs are \emph{a priori} chosen to have mean $\mu$.

Recall that given a Gaussian SCM $\mathcal{N}(\bm{\mu}, \bm{\Sigma})$, the adversary's goal is to remove from or add to the SCM learned by the modeler a set of edges using deception by omission. It may not be feasible to make such a modification while using a target SCM that is $\beta$-indistinguishable. In the case of linear Gaussian SCMs, given an adversarial DAG $\mathcal{G}_\alpha$, the adversary can: (i) determine the smallest $\beta$ such that there exists a distribution $\P_{\rvx; \vtheta_\alpha}$ whose moralized DAG is that of the moralization of $\mathcal{G}_\alpha$, and (ii) compute such a $\beta$-indistinguishable $\vtheta$. 

Both questions are answered by noting that the optimal $\beta$ and its corresponding distribution are respectively the objective value and the optimal parameter $\vtheta_\alpha$ for the optimization problem
\begin{equation*}
\label{eqn:best_beta}
\beta = \min_{\substack{\vtheta_\alpha \succ 0 \\ \vtheta_\alpha \in \mathcal{S}}} \KL( \mathcal{N}(\bm{\mu}, \bm{\Sigma}) \,\|\,  \mathcal{N}(\bm{\mu}, \bm{\Sigma}_\alpha )),
\end{equation*}
where $\mathcal{S}$ is the set of constraints corresponding to adding edges, i.e. $\left(\bm{\Theta}_\alpha\right)_{i,j} > \varepsilon$, or removing edges, i.e. $|\left(\bm{\Theta}_\alpha\right)_{i,j}| < \varepsilon$.

\begin{theorem}
\label{thm:best_beta}
Let $\mathcal{N}(\bm{\mu}, \bm{\Sigma}_\alpha)$ denote a distribution with the same mean as the true SCM and denote its precision matrix by $\bm{\Theta}_\alpha$. When $\mathcal{S}$ is a convex set, the optimal value of \eqref{eqn:best_beta} and the corresponding optimal parameters can be determined by solving a semidefinite program.
\end{theorem}

\begin{proof}
Writing the objective in terms of $\bm{\Theta}_\alpha$ gives
\begin{align}
\beta & = \min_{\substack{\bm{\Theta}_\alpha \succ 0 \\ \bm{\Theta}_\alpha \in \mathcal{S}}} \frac{1}{2} \left[ \log \left(\frac{\det \bm{\Sigma}_\alpha }{ \det \bm{\Sigma}}\right) - d + \textrm{Tr}(\bm{\Sigma}_\alpha^{-1} \bm{\Sigma}) \right] \nonumber \\
       & = \min_{\substack{\bm{\Theta}_\alpha \succ 0 \\ \bm{\Theta}_\alpha \in \mathcal{S}}} \frac{1}{2} \left[ \operatorname{Tr}(\bm{\Theta}_\alpha \bm{\Sigma}) - \log \det \bm{\Theta}_\alpha - \log \det \bm{\Sigma} - d \right].\label{eq:kl}
\end{align}
The constraint set is convex and $\log \det$ is concave on the set of positive definite matrices, so this is a convex optimization problem over the semidefinite cone, and $\beta$ can be determined numerically using an SDP solver. Further, any precision matrix $\bm{\Theta}_\alpha^\star$ that minimizes this objective tells us a corresponding distribution $\mathcal{N}(\bm{\mu}, \bm{\Sigma}_\alpha^\star)$ that achieves $\beta$-indistinguishability.
\end{proof}

Theorem~\ref{thm:gaussian_graph_structure} implies that $\bm{\Theta}_p$ reflects the graph structure of the moralized DAG of the true SCM, and that $\bm{\Theta}_\alpha$ reflects the graph structure of the moralized DAG of the adversarial SCM. If $\mathcal{G}_\alpha$ is obtained by dropping edges from or adding edges to $\mathcal{G}_p$, then its moralization is obtained by dropping edges from or adding edges to the moralization of $\mathcal{G}_p$. Thus when the constraint set $\mathcal{S}$ is chosen to correspond to dropping or adding edges in this way, Theorem~\ref{thm:best_beta} allows us to find an adversarial distribution within optimal distance $\beta$ of the true SCM, such that the moralized DAG of this distribution is the moralization of $\mathcal{G}_\alpha$. In general, this adversarial distribution may not be Markovian with respect to $\mathcal{G}_\alpha,$ so Theorem~\ref{thm:best_beta} provides a lower-bound on level of $\beta$-indistinguishability that can be achieved using an adversarial SCM with DAG $\mathcal{G}_\alpha$.

In some cases, we can find exactly the level of $\beta$-indistinguishability that can be achieved, along with the adversarial SCM that achieves that level of $\beta$-indistinguishability. In particular, consider the important case where $\mathcal{G}_\alpha$ is obtained by deleting a single edge coming into $\rvx_s$ from $\mathcal{G}_p$; for simplicity, we consider the case $\bm{\mu} = \bm{0}$. 
Among all SCMs that are Markov with respect to this $\mathcal{G}_\alpha,$ the closest in KL-divergence to $\P_{\rvx; \vtheta_p}$ is one in which the structural equation for all variables other than $\rvx_s$ remain unchanged, and for which the structural equation governing $\rvx_s$ is obtained by solving a convex optimization problem.
\end{comment}

In the case of linear Gaussian SCMs, Theorem~\ref{thm:optimal_adversarial_linear_gaussian_SCM} states that when $\mathcal{G}_\alpha$ is a subgraph of $\mathcal{G}_p$, we can find the optimal adversarial SCM in a closed form, in terms of the parameters of the true SCM.

\begin{proof}[Proof of Theorem~\ref{thm:optimal_adversarial_linear_gaussian_SCM}]
Let $\P_{\rvx; \vtheta}$ be Markovian with respect to $\mathcal{G}_\alpha$. Fix a $j$ in $1,\ldots,d$ and observe that the expected KL-divergence between $\P_{\rvx_j\mid \rvx_{\pa_j}; \vtheta_p}$ and $\P_{\rvx_j \mid \rvx_{\pa_j}; \vtheta}$ can be written in terms of an expected entropy and an expected cross-entropy term:
\begin{align*}
    \E_{\rvx_{\pa_j};\vtheta_p} \left[ \operatorname{D}_{\mathrm{KL}}\left( \P_{\rvx_j\mid \rvx_{\pa_j}; \vtheta_p} \,\|\, \P_{\rvx_j \mid \rvx_{\pa_j}; \vtheta} \right) \right] & \\
    & \kern -14em = \E_{\rvx_{\pa_j}; \vtheta_p} \left[ \E_{\rvx_j \mid \rvx_{\pa_j}; \vtheta_p} \left[ \ln \left( \frac{\p(\vx_j \mid \vx_{\pa_j}; \vtheta_p)}{\p(\vx_j \mid \vx_{\pa_j} ; \vtheta)}\right) \right] \right] \\
    & \kern -14em = \E_{\rvx_{\pa_j}; \vtheta_p} \left[ \E_{\rvx_j \mid \rvx_{\pa_j}; \vtheta_p} \left[ \ln ( \p(\vx_j \mid \vx_{\pa_j}; \vtheta_p) ) \right] \right] + \\
    & \kern -12em \E_{\rvx_{\pa_j}; \vtheta_p} \left[ \E_{\rvx_j \mid \rvx_{\pa_j}; \vtheta_p} \left[ - \ln( \p(\vx_j \mid \vx_{\pa_j} ; \vtheta) ) \right] \right]. \\
\intertext{Because the entropy term does not depend on $\vtheta$, we denote it with a constant $C_j$, and use the tower property of conditional expectation to continue further: }
    & \kern -14em = C_j + \E_{\rvx_{\pa_j \cup \{j\}}; \vtheta_p} \left[ -\ln( \p(\vx_j \mid \vx_{\pa_j} ; \vtheta) ) \right] \\
    & \kern -14em = C_j + \E_{\rvx_{\overline{\pa}_j \cup \{j\}; \vtheta_p}} \left[ -\ln( \p(\vx_j \mid \vx_{\overline{\pa}_j} ; \vtheta) ) \right] \\
    & \kern -14em = C_j + \E_{\rvx_{\overline{\pa}_j}; \vtheta_p} \left[ \E_{\rvx_j \mid \rvx_{\overline{\pa}_j}; \vtheta_p} \left[ - \ln( \p(\vx_j \mid \vx_{\overline{\pa}_j} ; \vtheta) ) \right] \right],
\intertext{ here, the second equation follows from observing that the integrand depends only on the variables in $\overline{\pa}_j$, and the others are integrated out. Now we reverse the procedure to obtain the expectation of the KL-divergence between $\P_{\rvx_j\mid \rvx_{\overline{\pa}_j}; \vtheta_p}$ and $\P_{\rvx_j \mid \rvx_{\overline{\pa}_j}; \vtheta}$:}
    & \kern -14em = C_j - D_j + \E_{\rvx_{\overline{\pa}_j};\vtheta_p} \left[ \operatorname{D}_{\mathrm{KL}}\left( \P_{\rvx_j\mid \rvx_{\overline{\pa}_j}; \vtheta_p} \,\|\, \P_{\rvx_j \mid \rvx_{\overline{\pa}_j}; \vtheta} \right) \right],
\end{align*}
where $D = \E_{\rvx_{\overline{\pa}_j}; \vtheta_p} \left[ \E_{\rvx_j \mid \rvx_{\overline{\pa}_j}; \vtheta_p} \left[ \ln ( \p(\vx_j \mid \vx_{\overline{\pa}_j}; \vtheta_p) ) \right] \right]$ is a cross-entropy and does not depend on $\vtheta.$ 

As a consequence, we have established that
\begin{multline}
\label{eqn:sum_of_kl}
\sum_{j=1}^d \E_{\rvx_{\pa_j};\vtheta_p} \left[ \operatorname{D}_{\mathrm{KL}}\left( \P_{\rvx_j\mid \rvx_{\pa_j}; \vtheta_p} \,\|\, \P_{\rvx_j \mid \rvx_{\pa_j}; \vtheta} \right) \right] = \\
C - D + \sum_{j=1}^d \E_{\rvx_{\overline{\pa}_j};\vtheta_p} \left[ \operatorname{D}_{\mathrm{KL}}\left( \P_{\rvx_j\mid \rvx_{\overline{\pa}_j}; \vtheta_p} \,\|\, \P_{\rvx_j \mid \rvx_{\overline{\pa}_j}; \vtheta} \right) \right],
\end{multline}
where $C$ and $D$ do not depend on $\vtheta$. Now we explicitly construct an adversarial $\vtheta$ which minimizes the right-hand side.

 Since $\P_{\rvx; \vtheta_p}$ is a linear Gaussian SCM with mean zero and covariance $\bm{\Sigma}$, the posterior conditional $\rvx_j \mid \rvx_{\overline{\pa}_j}; \vtheta_p$ is Gaussian~\cite{murphy2012machine},
 \[ 
 \rvx_j \mid \rvx_{\overline{\pa}_j}; \vtheta_p \sim \mathcal{N}(\mu_{j\mid \overline{\pa}_k}, \sigma^2_{j\mid \overline{\pa}_j}),
 \]
 with mean and variance
 \begin{align*}
     \mu_{j\mid \overline{\pa}_k} & = \left\langle\left(\bm{\Sigma}_{\overline{\pa}_j, \overline{\pa}_j}\right)^{-1} \bm{\Sigma}_{\overline{\pa}_j,j}, \rvx_{\overline{\pa}_j} \right\rangle, \text{ and } \\  
     \sigma^2_{j\mid \overline{\pa}_j} & = \bm{\Sigma}_{j,j} - \left \langle\bm{\Sigma}_{\overline{\pa}_j,j}, \left(\bm{\Sigma}_{\overline{\pa}_j, \overline{\pa}_j}\right)^{-1} \bm{\Sigma}_{\overline{\pa}_j,j}\right\rangle.
 \end{align*}
 Accordingly, when $\P_{\rvx; \vtheta_\alpha}$ is selected as the linear gaussian SCM satisfying the conditions in the statement of the theorem, (1) for each $j$, $\P_{\rvx_j \mid \rvx_{\overline{\pa}_j}; \vtheta_\alpha}$ is exactly $\P_{\rvx_j \mid \rvx_{\overline{\pa}_j}; \vtheta_p}$, and (2) $\P_{\rvx; \vtheta_\alpha}$ is Markov with respect to $\mathcal{G}_\alpha$.

This choice of $\vtheta_\alpha$ minimizes the right-hand side of~\eqref{eqn:sum_of_kl} with respect to $\vtheta$, so by Corollary~\ref{cor:adversarial_optimality_condition}, $\vtheta_\alpha$ solves 
 \[
 \argmin_{\vtheta\,:\, \P_{\rvx; \vtheta} \in \mathcal{D}} \operatorname{D}_{\mathrm{KL}}( \P_{\rvx ;\vtheta_p}  \,\|\, \P_{\rvx ; \vtheta}).
 \]
\end{proof}

\begin{comment}
\begin{theorem}
Given the true SCM $\rvx \sim \P = \mathcal{N}(0, \bm{\Sigma})$ with DAG $\mathcal{G}_p$, fix a variable $\rvx_s$ and let $\mathcal{G}_\alpha$ be an adversarial DAG obtained by deleting the edge between $\rvx_s$ and one of its parents in $\mathcal{G}$: in the notation of Corollary~\ref{cor:local_edge_deletion}, when $j \neq s$, $\pa_j = \overline{\pa}_j$, and when $j = s$, $\overline{\pa}_s \subsetneq \pa_s$ and $|\overline{\pa}_s| = |\pa_s| - 1.$ Because of the linear Gaussian nature of the true SCM,
\[
\vx_s \,|\, \vx_{\pa_s} \sim \mathcal{N}( \bm{\omega}^T \vx_{\pa_s}, \sigma^2)
\]
for some parameter vector $\bm{\omega}$ and some $\sigma^2 > 0$. 

There exists an adversarial linear Gaussian SCM $\P_\alpha$ that is Markovian with respect to $\mathcal{G}_\alpha$ and satisfies the bound
\[
\mathrm{D}_{\mathrm{KL}}(\P\,\|\, \P_\alpha) \leq \min_{\bm{\omega}_\alpha \, :\, (\bm{\omega}_\alpha)_{-\overline{\pa}_s} = 0 } \frac{1}{2\sigma^2} \operatorname{Tr}\left( \bm{\Sigma}_{\pa_s} \left(\bm{\omega} \bm{\omega}^T -2 \bm{\omega}\bm{\omega}_\alpha^T + \bm{\omega}_\alpha\bm{\omega}_\alpha^T \right) \right),
\]    
where $\bm{\Sigma}_{\pa_s}$ denotes the covariance matrix for $\rvx_{\pa_s}$ in the true SCM. Because $\bm{\Sigma}_{\pa_s}$ is positive semidefinite, this is a convex optimization problem.

This bound is achievable by deleting the desired causal relationship between $\rvx_s$ and one of its parent, optimizing over the weights of the other parents' contribution to $\rvx_s$, and keeping the exogenous noise level the same for $\rvx_s$ in the true and adversarial SCMs.
\end{theorem}

\begin{proof}
Write the causal factorization of the pdfs of the true and adversarial distributions as
$$
\p(\vx) = \prod_{j=1}^d p(\vx_j\,|\,\vx_{\pa_j}) \quad \text{ and } \p_\alpha(\vx) = \prod_{j=1}^d \p_\alpha(\vx_j\,|\,\vx_{\overline{\pa}_j}) 
$$
respectively, where $\p_\alpha(\vx_j\,|\,\vx_{\overline{\pa}_j}) := \p(\vx_j\,|\,\vx_{\pa_j})$ when $j\neq s$, and the (Gaussian) conditional distribution $\p_\alpha(\vx_s\,|\,\vx_{\overline{\pa}_s})$ is to be determined.

Then
\begin{align*}
\textrm{D}_{\text{KL}}(\P\,\|\, \P_\alpha) & = \E_{\P} \left[ \ln\left( \frac{\p(\vx)}{\p_\alpha(\vx)} \right) \right] =  
\E_{\P} \left[ \ln \left( \frac{p(\vx_s\,|\,\vx_{\pa_s})}{\p_\alpha(\vx_s\,|\,\vx_{\overline{\pa}_s})}\right) \right] := \E_{\P} \left[ R(\vx_s, \vx_{\pa_s}) \right],
\end{align*}
where the notation $R(\vx_s, \vx_{\pa_s})$ emphasizes that the integrand is a function of $\vx_s$ and its parents only. It follows that the $KL$-divergence can be computed by integrating over the ancestors of $\vx_s$, denoted by $\anc_s = \{s\} \cup \left\{ j \,|\, x_j \text{ is an ancestor of $\vx_s$ in $\mathcal{G}_p$} \right\}$:
\begin{align*}
D_{\text{KL}}(\P\,\|\, \P_\alpha) & = \E_\P [R(\vx_s, \vx_{\pa_s})]  = \E_{\rvx_{\anc_s}} \left[ R(\vx_s, \vx_{\pa_s}) \right] \\
& = \int \p_{\rvx_{\anc_s}}(\vx_{\anc_s}) \ln\left( \frac{\p(\vx_s \, |\, \vx_{\pa_s})}{\p_\alpha(\vx_s \,|\, \vx_{\overline{\pa}_s})} \right) d\vx_{\anc_s}.
\end{align*}

Beacuse it is a linear Gaussian SCM, the adversarial SCM satisfies
\[
\vx_s \,|\, \vx_{\overline{\pa}_s} \sim \mathcal{N}(\bm{\omega}_\alpha^T \vx_{\pa_s}, \sigma_\alpha^2),
\]
for some parameter vector $\bm{\omega}_\alpha$ and some $\sigma_\alpha^2 >0$, where $(\bm{\omega}_\alpha)_j = 0$ if $j \not\in \overline{\pa}_s$ by the assumption on $\mathcal{G}_\alpha$. It follows that
\begin{align*}
\ln\left( \frac{\p(\vx_s \, |\, \vx_{\pa_s})}{\p_\alpha(\vx_s \,|\, \vx_{\overline{\pa}_s})} \right)  & = \ln \left( 
\frac{ 
    \frac{1}{\sqrt{2\pi \sigma^2}} \exp\left(- \frac{|\vx_s - \bm{\omega}^T \vx_{\pa_s}|^2}{2 \sigma^2} \right)}{
  \frac{1}{\sqrt{2\pi \sigma_\alpha^2}} \exp\left(- \frac{|\vx_s - \bm{\omega}_\alpha^T \vx_{\pa_s}|^2}{2 \sigma_\alpha^2}\right)
}\right) \\
& = \ln\left( \frac{\sigma_\alpha}{\sigma} \right) + \frac{|\vx_s - \bm{\omega}_\alpha^T \vx_{\pa_s}|^2}{2 \sigma_\alpha^2} - \frac{|\vx_s - \bm{\omega}^T \vx_{\pa_s}|^2}{2 \sigma^2}.
\end{align*}

Take $\sigma_\alpha := \sigma$, so that the above log-ratio simplifies to
\begin{align*}
\ln \left( \frac{\p(\vx_s \, |\, \vx_{\pa_s})}{\p_\alpha(\vx_s \,|\, \vx_{\overline{\pa}_s})} \right)  & = \frac{1}{2\sigma^2} \left(|\vx_s - \bm{\omega}_\alpha^T \vx_{\pa_s}|^2 - |\vx_s - \bm{\omega}^T \vx_{\pa_s}|^2 \right) \\
& = \frac{1}{2\sigma^2} \left( |\bm{\omega}_\alpha^T \vx_{\pa_s}|^2 - |\bm{\omega}^T \vx_{\pa_s}|^2 + 2 (\bm{\omega} - \bm{\omega}_\alpha)^T \vx_{\pa_s} \vx_s \right).
\end{align*}
This facilitates further simplication of the KL-bound; namely,
\begin{align*}
D_{\text{KL}}(\P\,\|\, \P_\alpha) & = \int \p_{\rvx_{\anc_s}}(\vx_{\anc_s}) \ln\left( \frac{\p(\vx_s \, |\, \vx_{\pa_s})}{\p_\alpha(\vx_s \,|\, \vx_{\overline{\pa}_s})} \right) d\vx_{\anc_s} \\
& = \frac{1}{2\sigma^2} \int \p_{\rvx_{\anc_s}}(\vx_{\anc_s}) \left( |\bm{\omega}_\alpha^T \vx_{\pa_s}|^2 - |\bm{\omega}^T \vx_{\pa_s}|^2 + 2 (\bm{\omega} - \bm{\omega}_\alpha)^T \vx_{\pa_s} \vx_s \right) d\vx_{\anc_s} \\
& = \frac{1}{2\sigma^2} \int \p_{\rvx_{\anc_s}}(\vx_{\anc_s})  \left[ \operatorname{Tr}\left(\vx_{\pa_s} \vx_{\pa_s}^T (\bm{\omega}_\alpha \bm{\omega}_\alpha^T - \bm{\omega} \bm{\omega}^T)\right)  + 2\vx_s (\bm{\omega} - \bm{\omega}_\alpha)^T \vx_{\pa_s} \right] d\vx_{\anc_s}\\
& = \frac{1}{2\sigma^2} \left[ \operatorname{Tr}\left( \bm{\Sigma}_{\pa_s} (\bm{\omega}_\alpha \bm{\omega}_\alpha^T - \bm{\omega} \bm{\omega}^T) \right) + 2 (\bm{\omega} - \bm{\omega}_\alpha)^T \operatorname{Cov}(\vx_{\pa_s}, \vx_s)\right].
\end{align*}
Use the fact that $\vx_s = \bm{\omega}^T \vx_{\pa_s} + \varepsilon$ in the true SCM, where $\varepsilon \sim \mathcal{N}(0, \sigma^2)$, to compute the required covariance vector, 
\[
\operatorname{Cov}(\vx_{\pa_s}, \vx_s) = \E_{\rvx_{\pa_s}, \varepsilon} \left[ (\langle \bm{\omega}, \vx_{\pa_s} \rangle + \varepsilon) \vx_{\pa_s} \right] = \E_{\rvx_{\pa_s}}\left[ \langle \bm{\omega}, \vx_{\pa_s} \rangle \vx_{\pa_s} \right] = \bm{\Sigma}_{\pa_s} \bm{\omega}.
\]
This gives the final bound
\begin{align*}
D_{\text{KL}}(\P\,\|\, \P_\alpha) & \leq \frac{1}{2\sigma^2} \left[ \operatorname{Tr}\left( \bm{\Sigma}_{\pa_s} (\bm{\omega}_\alpha \bm{\omega}_\alpha^T - \bm{\omega} \bm{\omega}^T) \right) + 2 (\bm{\omega} - \bm{\omega}_\alpha)^T \bm{\Sigma}_{\pa_s} \bm{\omega} \right] \\
 & = \frac{1}{2\sigma^2} \left[ \operatorname{Tr}\left( \bm{\Sigma}_{\pa_s} (\bm{\omega}_\alpha \bm{\omega}_\alpha^T - \bm{\omega} \bm{\omega}^T) \right) + 2 \operatorname{Tr}\left(\bm{\Sigma}_{\pa_s} \bm{\omega}\left( \bm{\omega} - \bm{\omega}_\alpha \right)^T \right)  \right] \\
 & = \frac{1}{2\sigma^2} \operatorname{Tr}\left( \bm{\Sigma}_{\pa_s} \left(\bm{\omega} \bm{\omega}^T -2 \bm{\omega}\bm{\omega}_\alpha^T + \bm{\omega}_\alpha\bm{\omega}_\alpha^T \right) \right).
\end{align*}
This inequality is satisfied for any vector $\bm{\omega}_\alpha$ parameterizing the dependence of $\rvx_s$ on its parents $\rvx_{\overline{\pa}_s}$ in $\mathcal{G}_\alpha$, where $(\bm{\omega}_\alpha)_j = 0$ if $j \not\in \overline{\pa}_s$. By optimizing over such $\bm{\omega}_\alpha$, we find that there exists an adversarial SEM Markovian with respect to $\mathcal{G}_\alpha$ that has a KL distance satisfying 
\[
D_{\text{KL}}(\P\,\|\, \P_\alpha) \leq \min_{\bm{\omega}_\alpha \, :\, (\bm{\omega}_\alpha)_{-\overline{\pa}_s} = 0 } \frac{1}{2\sigma^2} \operatorname{Tr}\left( \bm{\Sigma}_{\pa_s} \left(\bm{\omega} \bm{\omega}^T -2 \bm{\omega}\bm{\omega}_\alpha^T + \bm{\omega}_\alpha\bm{\omega}_\alpha^T \right) \right),
\]
as claimed.  
\end{proof}
\end{comment}

\section{Proofs for Section~\ref{sxn:generalized_rejection_sampling}}
\label{sxn:proofs_for_rejection_sampling}
\begin{proof}[Proof of Lemma~\ref{lem:generalized_rejection_sampling}]
Fix an observation pattern $\vr \neq 0$ and the corresponding subset of observed features $\vx_o$. Observe that
\begin{align*}
\p_{\rvx_o \mid \rvr} (\vx_o \mid \vr) & = \frac{\p_{\rvr | \rvx_o}(\rv | \vx_o) \p_{\rvx_o}(\vx_o ; \vtheta_p) }{\p_{\rvr}(\vr)} \\
 & = \frac{\pi_\vr \Lambda_\vr(\vx_o)}{\p_\rvr(\vr) \Lambda_\vr^\star} \p_{\rvx_o}(\vx_o; \vtheta_p) \\
 & = \frac{\pi_\vr}{\p_\rvr(\vr) \Lambda_\vr^\star}\p_{\rvx_o}(\vx_o; \vtheta_\alpha) \\
 & \propto \p_{\rvx_o}(\vx_o; \vtheta_\alpha).
\end{align*}
The first equality uses Bayes' Theorem, the second uses the definition of the missingness mechanism for generalized rejection sampling (\eqref{eqn:generalized_rejection_sampler}), and the third uses the definition of $\Lambda_\vr(\vx_o).$ We have shown that, for each observation pattern $\vr \neq 0$, the density functions $\p_{\rvx_o \mid \rvr} (\cdot \mid \vr)$ and $\p_{\rvx_o}( \cdot \,; \vtheta_\alpha)$ are proportional, therefore the distributions are in fact equal, as claimed.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:rejection_sampling_global_maximizer}]
%First, observe that the modeler's objective function %(\eqref{eqn:modeler-objective}) satisfies
%\begin{align*}  
%    J(\vtheta) & = \E_{\rvr|\rvr\neq 0}\left[ \E_{\rvx_o|\rvr;\vtheta_p}\!\left[ \log \P_{\rvx_o;\vtheta}(\vx_o)\!\mid\! \rvr = \vr\right] \right] \\
%    & = \E_{\rvr|\rvr\neq 0}\left[ \E_{\rvx|\rvr;\vtheta_p}\!\left[ \log \P_{\rvx_o;\vtheta}(\vx_o)\!\mid\! \rvr = \vr\right] \right] \\
%    & = \E_{(\rvx, \rvr) \mid \rvr \neq 0; \vtheta_p} \log \P_{\rvx_o;\vtheta}(\vx_o) \\
%    & = \E_{\rvx;\vtheta_p} \left[ \E_{\rvr\mid \rvx, \rvr \neq 0} [ \log \P_{\rvx_o;\vtheta}(\vx_o) \mid \rvx = \vx] \right]
%\end{align*}
Recall that the modeler's objective (\eqref{eqn:modeler-objective}) is 
\[
J(\vtheta) = \E_{\rvr|\rvr\neq 0}\left[ \E_{\rvx_o|\rvr;\vtheta_p}\!\left[ \log \p_{\rvx_o;\vtheta}(\vx_o) \mid \rvr = \vr\right] \right].
\]
Fix a parameter $\vtheta \in \mathcal{D}$ and compute
\begin{align*}
J(\vtheta_\alpha)  - J(\vtheta) & =  \sum_{\vr \neq 0} \p_{\rvr\mid\rvr \neq 0}(\vr) \E_{\rvx_o\mid \rvr}\left[ \log \frac{\p_{\rvx_o}(\vx_o;\vtheta_\alpha)}{\p_{\rvx_o}(\vx_o; \vtheta)}\,\bigg|\, \rvr = \vr \right] \\
& = \sum_{\vr \neq 0} \p_{\rvr\mid\rvr \neq 0}(\vr) \E_{\rvx_o; \vtheta_\alpha}\left[ \log \frac{\p_{\rvx_o}(\vx_o;\vtheta_\alpha)}{\p_{\rvx_o}(\vx_o; \vtheta)}\,\bigg|\, \rvr = \vr \right] \\
& = \sum_{\vr \neq 0} \p_{\rvr\mid \rvr \neq 0}(\vr) \textrm{D}_{\textrm{KL}}(\P_{\rvx_o}(\cdot\,; \vtheta_\alpha)\,\|\, \P_{\rvx_o}(\cdot\,; \vtheta)) \\
& \geq 0.
\end{align*}
The second equality is justified by Lemma~\ref{lem:generalized_rejection_sampling}. This inequality shows that $\vtheta_\alpha$ is a global maximizer of the modeler's objective.
\end{proof}

\begin{proof}[Proof of Corollary~\ref{cor:attack_success_generalized_rejection_sampling}]
When the missingness distribution is constructed using the generalized rejection sampling of~\eqref{eqn:generalized_rejection_sampler}, Lemma~\ref{lem:generalized_rejection_sampling} states that 
the condition
\[\P_{\rvx_o \mid \rvr}(\cdot\,| \vr; \vtheta_p)=\P_{\rvx_o}(\cdot \,;\vtheta_\alpha)\]
is satisfied for all $\vr\neq 0$. Consequently, Theorem~\ref{thm:rejection_sampling_global_maximizer} applies and yields that $\vtheta_\alpha$ is a global maximizer of the modeler's objective, as claimed.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:generalized_rejection_sampling_missingness_bound}]
For all $\vr \neq 0$, it is the case that
\begin{align*}
\p_{\rvr}(\vr) & = \E_{\rvx;\vtheta_p} \left[ \p_{\rvr | \rvx}(\vr \mid \vx) \right] = \E_{\rvx;\vtheta_p} \left[ \pi_{\vr} \frac{\Lambda_\vr(\vx_o)}{\Lambda_\vr^\star} \right] \\
& = \frac{\pi_{\vr}}{\Lambda_{\vr}^\star} \E_{\rvx_o;\vtheta_p} \left[ \frac{\p_{\rvx_o}(\vx_o; \vtheta_\alpha)}{\p_{\rvx_o}(\vx_o; \vtheta_p)} \right] = \frac{\pi_{\vr}}{\Lambda_{\vr}^\star}.
\end{align*}
The first equality is the law of total probability, the second and third are justified by the definition of the missingness mechanism, and the forth follows from the fact that pdfs integrate to one.

Now the expected missingness rate can be computed as 
\begin{align*}
 \frac{1}{d}\E_{\rvr}[\ell_{\vr}] & = \p_{\rvr}(0) \frac{\ell_0}{d} + \frac{1}{d} \sum_{\vr \neq 0} \p_{\rvr}(\vr) \ell_{\vr} \\
  & = \left(1 - \sum_{\vr\neq 0} \p_{\rvr}(\vr) \right) + \frac{1}{d} \sum_{\vr\neq 0} \frac{\pi_{\vr}}{\Lambda_{\vr}^\star} \ell_{\vr} \\
  & = 1 - \sum_{\vr \neq 0} \frac{\pi_\vr}{\Lambda_\vr^\star} \left(1 - \frac{\ell_{\vr}}{d} \right).
\end{align*}
The first equality is an expansion of the expectation, the second uses the fact that $\ell_0 = d$ and the expression found for $\p_{\rvr}$, while the final equality is justified by algebra.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:localized_generalized_rejection_sampling}]
Fix an arbitrary $\vr$ satisfying $\p_\rvr(\vr) \neq 0$, and note that this implies that $\vr_{\overline{\mathcal{V}}}=1$. Fix a corresponding subset of observed features $\vx_o$. Observe that 
\begin{equation*}
\p_{\rvx_o\mid \rvr}(\vx_o \mid \vr; \vtheta_p) = \sum_{\vx_m} \p_{\rvx \mid \rvr}(\vx \mid \vr; \vtheta_p),
\end{equation*}
where the summation with respect to $\vx_m$ denotes summation over all the possible values of the unobserved features. It follows that 
\begin{align*}
\p_{\rvx_o\mid \rvr}(\vx_o \mid \vr; \vtheta_p) & = \sum_{\vx_m} \p_{\rvx \mid \rvr}(\vx \mid \vr; \vtheta_p) \\
& = \sum_{\vx_m} \p_{\rvx_{\overline{\mathcal{V}} \mid \mathcal{V}, \rvr}} (\vx_{\overline{\mathcal{V}}} \mid \vx_{\mathcal{V}}, \vr; \vtheta_p) \p_{\rvx_\mathcal{V} \mid \rvr}(\vx_{\mathcal{V}}\mid \vr; \vtheta_p) \\
& = \sum_{\vx_m} \p_{\rvx_{\overline{\mathcal{V}} \mid \mathcal{V}}} (\vx_{\overline{\mathcal{V}}} \mid \vx_{\mathcal{V}}; \vtheta_p) \p_{\rvx_\mathcal{V} \mid \rvr}(\vx_{\mathcal{V}}\mid \vr; \vtheta_p),
\end{align*}
where the last two equalities are justified by the chain rule and the fact that $\rvr \independent \rvx_{\overline{\mathcal{V}}} \mid \rvx_{\mathcal{V}}$. Now we apply the assumption that
\[
\P_{\rvx_{\overline{\mathcal{V}}} \mid \rvx_{\mathcal{V}}}( \cdot \mid  \cdot\,; \vtheta_\alpha) = \P_{\rvx_{\overline{\mathcal{V}}} \mid \rvx_{\mathcal{V}}}(\cdot \mid \cdot\, ; \vtheta_p),
\]
to see that
\begin{equation}\label{eqn:01}
\p_{\rvx_o\mid \rvr}(\vx_o \mid \vr; \vtheta_p) = \sum_{\vx_m} \p_{\rvx_{\overline{\mathcal{V}} \mid \mathcal{V}}} (\vx_{\overline{\mathcal{V}}} \mid \vx_{\mathcal{V}}; \vtheta_\alpha) \p_{\rvx_\mathcal{V} \mid \rvr}(\vx_{\mathcal{V}}\mid \vr; \vtheta_p).
\end{equation}

In fact, $\p_{\rvx_{\mathcal{V}} \mid \rvr }(\vx_{\mathcal{V}} \mid \vr; \vtheta_p) = \p_{\rvx_\mathcal{V}}(\vx_{\mathcal{V}}; \vtheta_\alpha)$. We use similar manipulations as those in the proof of Lemma~\ref{lem:generalized_rejection_sampling} to establish this fact. First, consider the case that $\vr_{\mathcal{V}} \neq 0$: 
\begin{align*}
\p_{\rvx_{\mathcal{V}} \mid \rvr }(\vx_{\mathcal{V}} \mid \vr; \vtheta_p) & = 
\frac{\p_{\rvr \mid \rvx_{\mathcal{V}}}(\rv \mid \vx_{\mathcal{V}}) \p_{\rvx_{\mathcal{V}}}(\vx_\mathcal{V}; \vtheta_p)}{\p_{\rvr}(\vr)} \\
& = \frac{1}{(2^{|\mathcal{V}|}-1) \Lambda \p_{\rvr}(\vr)} \Lambda(\vx_{\mathcal{V}}) \p_{\rvx_{\mathcal{V}}}(\vx_{\mathcal{V}};\vtheta_p) \\
& = \frac{1}{(2^{|\mathcal{V}|}-1) \Lambda \p_{\rvr}(\vr)} \p_{\rvx_\mathcal{V}}(\vx_\mathcal{V};\vtheta_\alpha) \\
& \propto \p_{\rvx_\mathcal{V}}(\vx_\mathcal{V};\vtheta_\alpha).
\end{align*}
The first equation is Bayes' Theorem, the second follows from the definition of the localized generalized rejection sampling missingness mechanism (\eqref{eqn:localized_generalized_rejection_sampling}), and the third uses the definition of $\Lambda(\vx_{\mathcal{V}})$. Since the pdfs $\p_{\rvx_{\mathcal{V}} \mid \rvr }( \cdot \mid \vr; \vtheta_p)$ and $\p_{\rvx_\mathcal{V}}(\cdot\,;\vtheta_\alpha)$ are proportional, they are in fact equal in the case that $\vr_{\mathcal{V}} \neq 0$. 

Similarly, when $\vr_{\mathcal{V}} = 0$, we have that
\begin{align*}
\p_{\rvx_{\mathcal{V}} \mid \rvr }(\vx_{\mathcal{V}} \mid \vr; \vtheta_p) & = \frac{1}{\p_{\rvr}(\vr)} \left(1 - \frac{\Lambda(\vx_{\mathcal{V}})}{\Lambda}\right) \p_{\rvx_{\mathcal{V}}}(\vx_{\mathcal{V}}; \vtheta_p) \\
& = \frac{1}{\p_{\rvr}(\vr)} \left( \p_{\rvx_{\mathcal{V}}}(\vx_{\mathcal{V}}; \vtheta_p) - \frac{1}{\Lambda} \p_{\rvx_{\mathcal{V}}}(\vx_{\mathcal{V}}; \vtheta_\alpha) \right),
\end{align*}
where the second equality follows from the definition of $\Lambda(\vx_{\mathcal{V}})$. Equivalently,
\begin{equation}\label{eqn:02}
\p_{\rvr}(\vr) \p_{\rvx_{\mathcal{V}} \mid \rvr }(\vx_{\mathcal{V}} \mid \vr; \vtheta_p) = \p_{\rvx_{\mathcal{V}}}(\vx_{\mathcal{V}}; \vtheta_p) - \frac{1}{\Lambda} \p_{\rvx_{\mathcal{V}}}(\vx_{\mathcal{V}}; \vtheta_\alpha).
\end{equation}
Observe that when $\vr_{\mathcal{V}}= 0$, by the definition of the localized generalized rejection sampling missingness mechanism,
\begin{align*}
\p_{\rvr}(\vr) & = \E_{\rvx;\vtheta_p} \p_{\rvr\mid\rvx}(\vr\mid\vx) \\
& = \E_{\rvx;\vtheta_p} \left( 1 - \frac{\Lambda(\vx_{\mathcal{V}})}{\Lambda} \right) \\
& = 1 - \frac{1}{\Lambda},
\end{align*}
where the last equation holds because $\E_{\rvx;\vtheta_p} \Lambda(\vx_{\mathcal{V}}) = 1.$ It follows from this observation and~\eqref{eqn:02} that $\p_{\rvx_{\mathcal{V}} \mid \rvr }(\vx_{\mathcal{V}} \mid \vr; \vtheta_p) = \p_{\rvx_{\mathcal{V}}}(\vx_{\mathcal{V}}; \vtheta_\alpha)$ when $\vr_{\mathcal{V}} = 0.$
Thus, as claimed, we have established that for any arbitrary $\vr$ satisfying $\p_\rvr(\vr) \neq 0$, it is the case that $\p_{\rvx_{\mathcal{V}} \mid \rvr }(\vx_{\mathcal{V}} \mid \vr; \vtheta_p) = \p_{\rvx_\mathcal{V}}(\vx_{\mathcal{V}}; \vtheta_\alpha)$.

Returning to~\eqref{eqn:01} and using this fact, we have that as claimed,
\begin{align*}
\p_{\rvx_o\mid \rvr}(\vx_o \mid \vr; \vtheta_p) & = \sum_{\vx_m} \p_{\rvx_{\overline{\mathcal{V}} \mid \mathcal{V}}} (\vx_{\overline{\mathcal{V}}} \mid \vx_{\mathcal{V}}; \vtheta_\alpha)p_{\rvx_\mathcal{V}}(\vx_{\mathcal{V}}; \vtheta_\alpha) \\
& = \sum_{\vx_m} \p_{\rvx}(\vx; \vtheta_\alpha) \\
& = \p_{\rvx_o}(\vx_o; \vtheta_\alpha)
\end{align*}
for any $\vr$ satisfying $\p_\rvr(\vr) \neq 0.$
\end{proof}

\begin{proof}[Proof of Corollary~\ref{cor:attack_success_localized_generalized_rejection_sampling}]
When the assumed conditions hold, Lemma~\ref{lem:localized_generalized_rejection_sampling} applies, so~\eqref{eqn:matched_conditional_distribution} holds. Then Theorem~\ref{thm:rejection_sampling_global_maximizer} applies and says that $\vtheta_\alpha$ is a global maximizer of the objective of the modeler.
\end{proof}


\begin{proof}[Proof of Corollary~\ref{cor:local_edge_deletion}]
Since the edges in $\mathcal{G}_\alpha$ are a subset of the edges of $\mathcal{G}_p$ and $\P_{\rvx;\vtheta_\alpha}$ is Markov relative to $\mathcal{G}_\alpha$, it is also Markov relative to $\mathcal{G}_p$.

Use the causal factorization of $\P_{\rvx;\vtheta_\alpha}$ relative to $\mathcal{G}_p$ to calculate the pdf of $\rvx_{\overline{\mathcal{V}}}$ conditional on $\rvx_\mathcal{V}$ under the adversarial distribution,
\begin{equation*}
	\begin{split}
		 &\p_{\rvx_{\overline{\mathcal{V}}} \mid \rvx_\mathcal{V}}(\vx_{\overline{\mathcal{V}}} \mid \vx_\mathcal{V} ; \vtheta_p) = 
		 \frac{\jp}
		 {\sum_{\vx_{\fu}}\jp}\\
		&=\frac{\cpd}{\cpd}\frac{\fp}{\sum_{\vx_{\fu}}\fp}\\
		&=\frac{\fp}{\sum_{\vx_{\fu}}\fp}\\
		&=\frac{\fa}{\sum_{\vx_{\fu}}\fa}\\
		&=\frac{\cpda}{\cpda}\frac{\fa}{\sum_{\vx_{\fu}}\fa}\\
		&=\frac{\ja}{\sum_{\vx_{\fu}}\ja}\\	
		&=\p_{\rvx_{\overline{\mathcal{V}}} \mid \rvx_\mathcal{V}}(\vx_{\overline{\mathcal{V}}} \mid \vx_\mathcal{V} ; \ta) 
	\end{split}
\end{equation*}

The first equality follows from the definition of conditional probability and the law of total probability. The second follows from the causal factorization and the fact that the variables indexed by $\nfu=\{s\}\cup \pa_s$ are not in the summation. The third equality is simple algebra, and the fourth follows from the assumption about the equality of the conditional marginals of the adversarial and true distributions. The last equality follows from the definition of conditional probability and the law of total probability. 

Because $\P_{\rvx_{\overline{\mathcal{V}}} \mid \rvx_{\mathcal{V}}}( \cdot \mid  \cdot\,; \vtheta_\alpha) = \P_{\rvx_{\overline{\mathcal{V}}} \mid \rvx_{\mathcal{V}}}(\cdot \mid \cdot\, ; \vtheta_p),$ holds, Corollary \ref{cor:attack_success_localized_generalized_rejection_sampling} applies.
\end{proof}

\begin{lemma}\label{lem:localized_generalized_rejection_sampling_missingness_bound}
Let $\ell_{\vr} = |\{j \mid \vr_j = 0\}|$ denote the amount of features missing in pattern $\vr$. When localized generalized rejection sampling is used on the variables $\mathcal{V}$, the expected missingness rate satisfies
\begin{align*}
\E_{\rvr}\left[\frac{|\{j\,|\,\rvr_j=0\}|}{d}\right]  & = 
 \left(1 - \frac{1}{\Lambda}\right)\frac{|\mathcal{V}|}{d} + \\
 & \kern -3em \frac{1}{\Lambda d }\cdot \frac{1}{\left(2^{|\mathcal{V}|} - 1\right)} \sum_{\vr:\vr_{\overline{\mathcal{V}}}=1, \vr_{\mathcal{V}} \neq \bm{0}} \ell_\vr,
\end{align*}
and consequently,
\begin{equation*}
\E_{\rvr}\left[\frac{|\{j\,|\,\rvr_j=0\}|}{d}\right] \leq \left(1 - \frac{1}{2 \Lambda} \right) \frac{|\mathcal{V}|}{d}.
\end{equation*}
\end{lemma}

\begin{proof}
To compute the expected missingness rate, first compute the probability of each observation pattern satisfying $\vr_{\overline{\mathcal{V}}}=\bm{1}$ and $\vr_{\mathcal{V}}\neq \bm{0}$,
\begin{align*}
    \p_{\rvr}(\vr) & = \E_{\rvx; \vtheta_p}[ \p_{\rvr\mid\rvx}(\vr\mid\vx)] = \E_{\rvx; \vtheta_p}\left[ \frac{\Lambda(\vx_\mathcal{V})}{\Lambda} \frac{1}{2^{|\mathcal{V}|} - 1} \right]  \\
    & = = \frac{1}{(2^{|\mathcal{V}|} - 1) \Lambda} \E_{\rvx_{\mathcal{V};\vtheta_p}}[ \Lambda(\vx_\mathcal{V})] \\
    & = \frac{1}{(2^{|\mathcal{V}|} - 1) \Lambda} \E_{\rvx_{\mathcal{V};\vtheta_p}}\left[ \frac{\p_{\rvx_{\mathcal{V}}}(\vx_{\mathcal{V}}; \vtheta_\alpha)}{\p_{\rvx_{\mathcal{V}}}(\vx_{\mathcal{V}}; \vtheta_p)} \right] 
    =  \frac{1}{(2^{|\mathcal{V}|} - 1) \Lambda}.
\end{align*}
When $\vr_{\overline{\mathcal{V}}}=\bm{1}$ and $\vr_{\mathcal{V}}= \bm{0}$, then similarly
\begin{align*}
    \p_{\rvr}(\vr) & = \E_{\rvx; \vtheta_p}[ \p_{\rvr\mid\rvx}(\vr\mid\vx)] = \E_{\rvx; \vtheta_p}\left[ 1 - \frac{\Lambda(\vx_\mathcal{V})}{\Lambda} \right]  \\
    & = = 1 - \frac{1}{\Lambda} \E_{\rvx_{\mathcal{V};\vtheta_p}}[ \Lambda(\vx_\mathcal{V})]\\
    & = 1 - \frac{1}{\Lambda} \E_{\rvx_{\mathcal{V};\vtheta_p}}\left[ \frac{\p_{\rvx_{\mathcal{V}}}(\vx_{\mathcal{V}}; \vtheta_\alpha)}{\p_{\rvx_{\mathcal{V}}}(\vx_{\mathcal{V}}; \vtheta_p)} \right] 
    = 1 - \frac{1}{\Lambda}.
\end{align*}
Thus the expected missingness rate can be calculated as 
\begin{equation*}
    \E_{\rvr}\left[\frac{|\{j\,|\,\rvr_j=0\}|}{d}\right] = \p_{\rvr}(\bm{0}) \frac{|\mathcal{V}|}{d} +  
    \frac{1}{d} \sum_{\vr\,:\, \vr_{\overline{\mathcal{V}}} = \bm{1}, \vr_{\mathcal{V}} \neq \bm{0} } \p_{\rvr}(\vr) \E [ \ell_\vr],
\end{equation*}
where $\ell_{\rv}$ is defined as in Lemma~\ref{lem:generalized_rejection_sampling_missingness_bound}. Inserting the expressions for $\p(\vr)$ from above establishes the first claim of this lemma,
\begin{align}
\label{eqn:first_claim}
\E_{\rvr}\left[\frac{|\{j\,|\,\rvr_j=0\}|}{d}\right] & = 
 \left(1 - \frac{1}{\Lambda}\right)\frac{|\mathcal{V}|}{d} + \\
 & \kern -3em \frac{1}{\Lambda d }\cdot \frac{1}{\left(2^{|\mathcal{V}|} - 1\right)} \sum_{\vr:\vr_{\overline{\mathcal{V}}}=1, \vr_{\mathcal{V}} \neq \bm{0}} \ell_\vr.
\end{align}
The second claim follows from the observation that each coordinate in $\rv_{\mathcal{V}}$ can be viewed as the result of flipping a fair coin. This implies that the average of the $\ell_{\rv}$ on the right-hand side of this equation is the expected number of failures in $|\mathcal{V}|$ independent experiments, each with probability $\tfrac{1}{2}$ of success, conditioned on the fact that there is at least one success. That is,
\begin{align*}
\frac{1}{\left(2^{|\mathcal{V}|} - 1\right)} \sum_{\vr:\vr_{\overline{\mathcal{V}}}=1, \vr_{\mathcal{V}} \neq \bm{0}} \ell_\vr & = \E_{b \sim \operatorname{Bin}(|\mathcal{V}|, \frac{1}{2})}[|\mathcal{V}| -  b \mid b > 0] \\
& \kern -6em = |\mathcal{V}| - \frac{\E[b]}{\P(b \neq 0)} \leq |\mathcal{V}| - \E[b]
 = \frac{|\mathcal{V}|}{2}.
\end{align*}
Using this estimate in \eqref{eqn:first_claim} gives, as claimed,
\begin{align*}
    \E_{\rvr}\left[\frac{|\{j\,|\,\rvr_j=0\}|}{d}\right]  \leq 
 \left(1 - \frac{1}{\Lambda}\right)\frac{|\mathcal{V}|}{d} + \frac{1}{2} \frac{|\mathcal{V}|}{\Lambda d} = \left(1 - \frac{1}{2 \Lambda} \right) \frac{|\mathcal{V}|}{d}.
\end{align*}
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{WEM}\label{app:wem}

We have provided the WEM algorithm below. As discussed the main difference to EM algorithm is the missigness weights introduced. 

\subsection{Maximization step for exponential family}
When $\P_{\rvx;\vtheta}$ is in an exponential family, the weighed maximization step has a simplified form. Let $T: \R^d\rightarrow \R^k$ denote $k$-dimensional sufficient statistics such that 
\[
\p_{\rvx}(\vx;\vtheta)=h(\vx)\exp[\vtheta^T T(\vx)-A(\vtheta)],
\] 
\cite{murphy2012machine}. Given a $\vphi$ and an estimate $\vtheta^{t-1}$, we define the weighted conditional sufficient statistic as
\[
\tilde{\T}(\mathcal{S})\defeq \sum_{i=1}^N \sum_{\vr\neq 0} \omega_{i,r}(\vphi) \E_{\rvx; \vtheta^{t-1}}[T(\vx) \mid \rvx_{o}=\vx_{o}^{(i)}].
\]
One can show that the maximization step of WEM (Eq. \ref{eq:wem}) i.e.

\[
	\vtheta^t = \argmax_{\vtheta} \sum_{i=1}^N \sum_{\vr\neq 0}\omega_{i,r}(\vphi)
	\E_{\rvx;\vtheta^{t-1}}\left[\log \P_{\rvx}(\rvx; \vtheta) \mid \rvx_{o}=\vx_{o}^{(i)}\right]
\]

is equivalent to 

\begin{equation}\label{eq:suff}
	\vtheta^t = \argmax_{\vtheta} \vtheta^T \tilde{T}(\mathcal{S})-N \cdot A(\vtheta)
\end{equation}

This optimization problem in Eq. \ref{eq:suff} has the same form for the Maximum Likelihood Estimation (MLE) with the compeltely observed data. The only difference lies in the sufficient statistics. Therefore, the same optimization procedure used for MLE estimation with fully observed data can be used with in maximization step of the WEM algorithm by replacing the original sufficient statistics with the weighted conditional sufficient statistics. This has been previously observed for the maximization step of the original EM algorithm\cite{dempster}. In our case we have an additional expectation with respect to the missing data patterns.

%Heuristically, I have derived the new update equations as follows \footnote{I think at least as $N$ goes to infinity the equations are correct}:

For the MVN distribution, the sufficient statistics is given by $\T(\vx)=(\vx,\vx \vx^T)^T$, and the update equations become:

\begin{equation}
	\begin{split}
		\mu_t &= \frac{\tilde{\T}(\data)_1}{N}=\frac{1}{N} \sum_{i=1}^N \sum_{\vr\neq 0} \omega_{i,r}(\vphi) \E_{\rvx; \vtheta^{t-1}}[\rvx \mid \rvx_{o}=\vx_{o}^{(i)}]\\
		\Sigma_t &= \frac{\tilde{\T}(\data)_2}{N}-\mu_t(\mu_t)^T\\
		&=	\frac{1}{N} \sum_{i=1}^N \sum_{\vr\neq 0} \omega_{i,r}(\vphi) \E_{\rvx; \vtheta^{t-1}}[\rvx \rvx^T \mid \rvx_{o}=\vx_{o}^{(i)}]-\mu_t(\mu_t)^T
	\end{split}
\end{equation}

As discussed, those equations are similar to EM update equations (See chapter 11.6.1.3 in \cite{murphy2012machine}) with the additional inner summation. The conditional expectations can be calculated using the Multivariate Gaussian update equations (See chapter 4.3.1 in \cite{murphy2012machine}).

\section{Experiment Details}

\subsection{Gaussian SCM, I}\label{app:scm1}
$\mB=\begin{bmatrix}
	0 & -.9 & -.8\\
	0 & 0 & 0\\
	0 & 0 & 0
\end{bmatrix}$, equal variance with $\sigma=1$. $N=1000$. 
\subsection{Gaussian SCM, II}\label{app:scm2}

We use equal variance with $\sigma=1$.

$\mB =\begin{bmatrix}
	0.  & -0.54& 0.  & 1.15& 0.  & 0. \\
	0.  & 0.  & 0.4& 0.  & 0.  & 0. \\
	0.  & 0.  & 0.  &-1.43&-0.9 & 1.29\\
	0.  & 0.  & 0.  & 0.  & 0.  & 0.  \\
	0.  & 0.  & 0.  & 0.  & 0.  & 0. \\
	0.  & 0.  & 0.  & 0.  & 0.  & 0. \\
\end{bmatrix}$

To reduce the number of missing data we used a variation of the local rejection sampling Lem \ref{lem:localized_generalized_rejection_sampling}. Specificially, when a sample is accepted instead of uniformly distribution missing data patttern, we constrained it to be all or none i.e. 

\begin{equation}
	\P_{\rvr|\rvx}(\vr|\vx) = \begin{cases}
		 \frac{\Lambda(\vx_{\mathcal{V}})}{\Lambda} & \text{ if } \vr_{\overline{\mathcal{V}}}=1 \text{ and } \vr_{\mathcal{V}} = 1 \\
		1 - \frac{\Lambda(\vx_{\mathcal{V}})}{\Lambda} & \text{ if } \vr_{\overline{\mathcal{V}}}=1 \text{ and } \vr_{\mathcal{V}} = 0 \\
		0 & \text{ otherwise}
	\end{cases}.
\end{equation}

In addition, the maximum density ratio $\Lambda$ is selected as maximum density ratio over the observed samples.

\subsection{Setup for \namenn } \label{app:nn}
% Table generated by Excel2LaTeX from sheet 'edit'

 We have used Tensorflow v2.4. \cite{tensorflow} for implementation. We have implemented a Keras model with a custom training loop which includes the WEM Algorithm (Alg. \ref{alg:wem}) as subroutine. In our experiments, we have used $K=5$, random initializations for the \namenn which are sampled using \text{make\_spd\_matrix} function of \cite{scikit-learn} and scaled such that the diagonal entries match the empirical variances. We used $\epsilon=1e-5$ for the stopping criterion of WEM. 
 
 \subsection{NN parameters}
 
 \begin{itemize}
 	\item Weight initialization: Tensorflow default
 	\item Custom loss function as defined in Algorithm \ref{alg:nn}:
 	\[\sum_{k=1}^K\ell (\ttil_k, \ta,\vphi,\lambda)\]
 	\item Stopping criterion
 	\begin{enumerate}
 		\item Sachs: Fixed 300 epochs
 		\item Gaussian SCM,I: early stopping (restore best, min change = 1e-4, patience =10,monitor=loss function of the final initialization in WEM)
 		 	\end{enumerate}
 		\item Optimizer: Adam, 	learning rate = 1e-3 (Sachs ), 1e-2 (Gaussian SCM,I) 

 \end{itemize}

\subsection{Hyper-parameters for the Causal Discovery Algorithms}
\subsubsection{NOTEARS}
We used the code\footnote{https://github.com/xunzheng/notears/tree/master/notears} provided by the authors of \cite{notears} and used didn't change the hyper-parameters i.e. 

\begin{itemize}
	\item \text{max\_iter}=100, 
	\item \text{h\_tol}=1e-8, 
	\item \text{rho\_max}=1e+16, 
	\item \text{w\_threshold}=0.
\end{itemize}
\subsubsection{PC, missPC}
We used package causal-learn available at \footnote{https://github.com/py-why/causal-learn}. We used the hyper-parameters used an example test file:
For PC:
\begin{itemize}
	\item \text{pc\_alpha}=0.01
	\item \text{indep\_test}=``fisherz''
	\item \text{uc\_priority}=-1.
\end{itemize} 

For missPC:
\begin{itemize}
	\item \text{pc\_alpha}=0.01
	\item \text{indep\_test}=``mv\_fisherz''
	\item \text{uc\_priority}=-1.
	\item mvpc=True
\end{itemize} 

\subsubsection{missDAG}\label{app:init}
Algorithm is provided in Alg. \ref{alg:em}.

\begin{itemize}
	\item Initialization: Five different initialization schemes for the covariance matrix: using a diagonal matrix scale to match the estimated variances (``Emp. Diag.''),
	using an identity matrix (``Ident.''), the ground truth covariance matrix (``True''), a scaled random covariance matrix Random(*)\footnote{Generated using the \texttt{make\_spd\_matrix} function of scikit-learn and scaled to match the empirical variances.}, and a scaled inverse Wishart random matrix IW(*) \footnote{It uses the \texttt{make\_spd\_matrix} function of scikit-learn for the prior parameter.}.	
	\item Variance equality: equal variance (Gaussian SCM I, and II), non-equal variance (Sachs dataset)
	\item  Stopping criterion: $\epsilon=1e-5$.
\end{itemize}



\subsection{MissDAG Algorithm}

We have derived our equations and implemented our version based on the description in \cite{missdag} as their code was unavailable.

MissDAG uses the EM algorithm but optimizes the maximization step with a DAG constraint. Let N i.i.d. samples from $P_{X;\tr}$ and $P_{R\mid X}$ are denoted by $x^{(1)},\dots, x^{(N)}$ and $R^{(1)},\dots, R^{(N)}$ respectively. We denote $o^{i}=\{j:R^{(i)}_j=1\}$ and its complement as $-o^{i}$. Following Eq. xx \cite{missdag}, given $\vtheta^{t-1}$ (parameters from the previous step),  the maximization step of the EM algorithm is


\begin{equation}\label{eq:em}
	\vtheta^t = \argmax_{\vtheta\in \mathcal{D}} \sum_{i=1}^N 
	\E_{\rvx;\vtheta^{t-1}}\left[\log \P_{\rvx}(\rvx; \vtheta) \mid \rvx_{o^i}=\vx_{o^i}^{(i)}\right]
\end{equation}

 Under the zero mean-Gaussian SCM with equal variance noise assumption the likelihood has a simple form (see \cite{golem} appendix ) and because Gaussian SCM is an exponential family distribution the Eq. \ref{eq:em} also has a simple form. Let $\hat{\mathcal{S}}=\{\vx_{o^1}^{(1)},\dots,\vx_{o^N}^{(N)}\}$, we denote the aggregate sufficient statistics as

\begin{equation}\label{eq:suffhat}
	\hat{\T}(\hat{\mathcal{S}})\defeq \sum_{i=1}^N \E_{\rvx; \vtheta^{t-1}}[\rvx\rvx^T \mid \rvx_{o^i}=\vx_{o^i}^{(i)}]
\end{equation}
Given $W\in \real^{d\times d}$, let $W_j$ denotes the j'th column and similarly $\hat{\T}(\hat{\mathcal{S}})_j$ denotes the j'th column of the aggregate sufficient statistic. It can be shown that $Eq. \ref{eq:em}$ is equals to 

\begin{equation} \label{eq:missdag}
	\begin{split}
		W^t &= \argmin_{\mB\in \mathcal{D}} \sum_{j=1}^d  \hat{\T}(\hat{\mathcal{S}})_{j,j}-2\inner{\mB_j}{\hat{\T}(\hat{\mathcal{S}})_j}+ \inner{\mB_j}{\hat{\T}(\hat{\mathcal{S}})\mB_j} \\
	\end{split}
\end{equation}

For $\sigma$ is given under the equal variance assumption as 
\begin{equation}\label{eq:miss1}
			\sigma^t = \dfrac{1}{Nd}\sum_{j=1}^d  \hat{\T}(\hat{\mathcal{S}})_{j,j}-2\inner{\mB_j^t}{\hat{\T}(\hat{\mathcal{S}})_j}+ \inner{\mB_j^t}{\hat{\T}(\hat{\mathcal{S}})\mB_j^t}
\end{equation}
Under the non-equal variance assumption it is 
\begin{equation}\label{eq:miss2}
	\sigma^t_j = \dfrac{1}{N}\hat{\T}(\hat{\mathcal{S}})_{j,j}-2\inner{\mB_j^t}{\hat{\T}(\hat{\mathcal{S}})_j}+ \inner{\mB_j^t}{\hat{\T}(\hat{\mathcal{S}})\mB_j^t}
\end{equation}

Following \cite{missdag} we used the NOTEARS package to solve Eq. \ref{eq:missdag}. We implemented Eq. \ref{eq:missdag} as a custom loss function and provided its gradient with the python package Autograd \cite{autograd}. The empirical likelihood is given by:

\[\hat{J}(\theta)=\sum_{i=1}^N\log \P_{\rvx_{o^i}}(\vx_{o^i}^{(i)}; \vtheta) \]

The overall missDAG algorithm is given as follows:

\begin{algorithm}[tb]
	\caption{Our implementation of the MissDAG Algorithm \cite{missdag}. }
	\label{alg:em}
	
	\begin{algorithmic}
		\STATE {\bfseries Input: $ \epsilon, \hat{\data}$ }
		%		\State $\tat{0}\leftarrow\tr$
		\STATE $t\leftarrow 1$
		\WHILE{$\hat{J}(\vtheta^{(t)})-\hat{J}(\vtheta^{(t-1)})\geq \epsilon |J(\vtheta^{(t-1)},\bm{\phi})|$} 
		\STATE $\hat{\T} \leftarrow $ Eq. \ref{eq:suffhat} using  $\vtheta^{(t-1)},\hat{\mathcal{S}}$
		\STATE $\mB^t \leftarrow $ Eq. \ref{eq:missdag} via NOTEARS using $\hat{\T}$
		\STATE $\sigma^t \leftarrow $ Eq. \ref{eq:miss1} or Eq. \ref{eq:miss2} using $\mB^t,\hat{\T}$
		\STATE $\Sigma^t \leftarrow (I-\mB)^{-1}D(\sigma^t)(I-\mB)^{-T}$
		\STATE $\vtheta^t=\Sigma^t$
		\STATE $t\leftarrow t+1$
		\ENDWHILE
		\STATE $\that \leftarrow \vtheta^{t-1}$
		\STATE {\bfseries Output: $\that$} 
	\end{algorithmic}
\end{algorithm}

\section{Additional Results for the Sachs Dataset}\label{app:sachs}

\begin{figure}[H]
	\centering
	\includegraphics[width=1.\columnwidth]{sachs/loss.png}
	\caption{Model training curves for \namenn. Loss function over epochs (left). $\%$ missigness and $\%$ fully missing rows in the masked columns (in $\midx$).}
	\label{fig:loss}
\end{figure}
\begin{figure*}
	\begin{subfigure}[\namenn]{}
		\includegraphics[width=1.\textwidth]{sachs/em.png}
	\end{subfigure}
	\begin{subfigure}[MCAR]{}
		\includegraphics[width=1.\textwidth]{sachs/mcar.png}
	\end{subfigure}
	\caption{Results for Sachs dataset. Each scatter plot is a different initialization. Left to right: $\text{D}_{\text{KL}}(\P_{\rvx;\that} \| \P_{\rvx;\ta})$ vs $\text{D}_{\text{KL}}(\P_{\rvx;\that} \| \P_{\rvx;\tr})$; distribution of HD($\hat{\mathcal{G}},\mathcal{G}_{p}$); distribution of HD($\hat{\mathcal{G}},\ga$); adversarial success.}
\end{figure*}


\end{document}
\endinput
%%
%% End of file `sample-authordraft.tex'.

